Fully Dynamic Set Cover via Hypergraph Maximal Matching: An Optimal Approximation Through a Local Approach

In the (fully) dynamic set cover problem, we have a collection of $m$ sets from a universe of size $n$ that undergo element insertions and deletions; the goal is to maintain an approximate set cover of the universe after each update. We give an $O(f^2)$ update time algorithm for this problem that achieves an $f$-approximation, where $f$ is the maximum number of sets that an element belongs to; under the unique games conjecture, this approximation is best possible for any fixed $f$. This is the first algorithm for dynamic set cover with approximation ratio that {exactly} matches $f$ (as opposed to {almost} $f$ in prior work), as well as the first one with runtime \emph{independent of $n,m$} (for any approximation factor of $o(f^3)$). Prior to our work, the state-of-the-art algorithms for this problem were $O(f^2)$ update time algorithms of Gupta et al. [STOC'17] and Bhattacharya et al. [IPCO'17] with $O(f^3)$ approximation, and the recent algorithm of Bhattacharya et al. [FOCS'19] with $O(f \cdot \log{n}/\epsilon^2)$ update time and $(1+\epsilon) \cdot f$ approximation, improving the $O(f^2 \cdot \log{n}/\epsilon^5)$ bound of Abboud et al. [STOC'19]. The key technical ingredient of our work is an algorithm for maintaining a {maximal} matching in a dynamic hypergraph of rank $r$, where each hyperedge has at most $r$ vertices, which undergoes hyperedge insertions and deletions in $O(r^2)$ amortized update time; our algorithm is randomized, and the bound on the update time holds in expectation and with high probability. This result generalizes the maximal matching algorithm of Solomon [FOCS'16] with constant update time in ordinary graphs to hypergraphs, and is of independent merit; the previous state-of-the-art algorithms for set cover do not translate to (integral) matchings for hypergraphs, let alone a maximal one. Our quantitative result for the set cover problem is [...]

==> random.tex <==

{\bf 3.2~ Epochs.~}
Given any sequence of edge updates, an edge $(u,v)$ may become matched or unmatched by the algorithm at different update steps.
The entire lifespan of an edge $(u,v)$ consists of a sequence of \emph{epochs}, which refer to the maximal time intervals in which the edge is matched,
separated by
%\emph{anti-epochs}, which refer to
%the maximal continuous
the maximal time intervals in which the edge is unmatched.
(This notion of epoch was introduced in \cite{BGS11}.)  % will be ued in our analysis.
%Following \cite{BGS11}, we use the concept of \emph{epochs}.
%\begin{definition} \cite{BGS11}
Formally, let $e = (u,v)$ be any matched edge at some time step $l$.
The \emph{epoch} $\cE(e,l)$ corresponding to edge $e$ at time $l$ refers to the maximal time interval containing $l$
during which the edge $(u,v)$ is matched.
%[[S: should stress that this object is not just a time interval, but rather
%a pair -- an epoch refers to that edge within the relevant time interval, or to all the copies of that edge,
%but not to a time interval standing alone]]
%\end{definition}
%\ignore{
%An epoch $\cE(e,l)$ is not just a time interval, but rather an object describing a \emph{specific edge} within that time interval.
%In particular, for any two distinct (matched) edges $e$ and $e'$ and any time $l$, the respective epochs $\cE(e,l)$ and $\cE(e',l)$ refer to different objects.
%On the other hand, for two distinct times $l$ and $l'$ and some edge $e$, it is possible that the respective epochs $\cE(e,l)$ and $\cE(e,l')$
%refer to the same object.
%}
By Invariant \ref{exception}(c),  the endpoints of a matched edge are of the same level, and this level remains unchanged.  % throughout the entire epoch.
We   henceforth define the level of an epoch to be the level of the corresponding edge.

%The entire lifespan of an edge $(u,v)$ consists of a sequence of its epochs, separated by the maximal continuous time intervals
%when $(u,v)$ is unmatched, which we call \emph{anti-epochs}.

Any edge update that does not change the matching is processed by our algorithm in constant time.
However, an edge update that changes the matching may trigger the creation of some epochs and the termination of some  epochs.
% whose computation costs
%may be very large.
The computation cost of creating or terminating an epoch by the algorithm may be large. Moreover, the number of epochs created and terminated due to
a single edge update may be large by itself. Hence an amortized analysis is required.
%The computation performed at an arbitrary update step $t$ may be very large,
%which
%and there is no hope for bounding it in the worst-case.
Following the amortization scheme of \cite{BGS11},
%we employ the following two-step amortization scheme.
%[[S: This is not what we actually do, which is to combine them messily]]
%\begin{enumerate}
%\item In the first step (Section \ref{sec:dist}),
we re-distribute the total computation performed at any  step $l$ among the epochs created or terminated at step $l$.
Specifically, let $\cE_1 = \cE(e_1,l),\ldots,\cE_j = \cE(e_j,l)$ (resp., $\cE'_1 = (e'_1,l),\ldots,\cE'_k = (e'_k,l)$) be the epochs created (resp., terminated) at update step $l$, and let $C_{create}(\cE_1),\ldots,C_{create}(\cE_j)$ (resp., $C_{term}(\cE'_1),\ldots,C_{term}(\cE'_k)$) be the respective
computation costs charged to the creation (resp., termination) of these epochs.
Then we re-distribute the total computation cost performed at update step $l$, denoted by $C^{(l)}$,
to the respective epochs so that $C^{(l)} = \sum_{i=1}^j C_{create}(\cE_i) + \sum_{i=1}^k C_{term}(\cE'_i)$.
%The basic idea here is to over-charge the cost of creating or terminating an epoch, in order to express the total runtime of the algorithm as
%the sum of creation and termination costs over the various epochs.

%\vspace{-6pt}
%\begin{corollary}
%\begin{claim} \label{levelepoch}
Notice that any epoch created by Procedures $\ins$ or $\detr$ is of level 0.
On the other hand, we argue that any epoch created by Procedure $\rand$ is of level at least 1.
%\end{claim}
%\vspace{-6pt}
%\begin{proof}
%\end{corollary}
%(1) Immediate.
Indeed, consider a vertex $v$ that is handled via Procedure $\rand(v)$. First note that $\dout(v) \ge 5^{\ell_v+1} \ge 1$.
By Invariant \ref{exception}, $\ell_v \ge 0$.
By the description of Procedure $\rand(v)$ and Lemma \ref{rand_basic}(1),
we conclude that any epoch created by this procedure is of level at least $\ell^* > \ell_v$.
%So any epoch created by Procedure $\rand$ is of level greater than 0.]]
%\end{proof}
Applying now Lemma \ref{rand_basic}, we derive the following corollary.
%\vspace{-3pt}
\begin{corollary} \label{Ob:basic}
For any epoch at level $\ell > 0$, initiated by vertex $v$ and corresponding to edge $(v,w)$:
%\begin{itemize}
\vspace{2pt}\\(1) The out-degree of $v$ at the time the epoch is created is at least $5^{\ell}$ and less than $5^{\ell+1}$,
though the out-degree of $w$ at that time
% (after the call to $\setlvl(w,\ell)$)
may be significantly smaller or larger than $5^{\ell}$.
\vspace{2pt}\\(2) $w$ is chosen as $v$'s mate uniformly at random among all outgoing neighbors of $v$ at that time,
so the corresponding edge $(v,w)$ becomes matched with probability at most $1/5^{\ell}$.  % among all outgoing neighbors of $u$ at that stage.
%\end{itemize}
\end{corollary}

%On the other hand, when charging to the termination cost of some epoch, the idea is to ``charge the past''.
%That is, we charge based on past edge deletions that are expected to occur.
%\end{enumerate}
\vspace{7pt}
\noindent{\bf 3.3~ Re-distributing the computation costs to epochs.~}
%\label{sec:dist}
By re-distributing the total computation cost of the update algorithm to the various epochs, we can \emph{visualize} the entire update algorithm as a sequence of creation and termination of these epochs.
%We will thus analyze the number of epochs created and terminated during the algorithm as well as the computation costs associated with each epoch.
%In what follows
The computation cost associated with an epoch at level $\ell$ (hereafter,  \emph{level-$\ell$ epoch}) includes both its creation cost and its termination cost.

The following lemma plays a central role in our analysis.
Although a similar lemma was proved in \cite{BGS11}, our proof is inherently different than the corresponding proof of \cite{BGS11}.
%The proof is omitted due to space constraints, but appears in the full version \cite{Solom16}.
%Our goal is to re-distribute  the total computation cost
%to the various epochs in such a way that the creation and termination costs associated with an epoch of level $\ell$
%will be bounded by $O(5^{\ell})$.
%[[S: Explain a few more things, and then derive the following corollary !!rather than lemma]]
%\vspace{-1pt}
\begin{lemma} \label{basiccost}
The total computation cost of the update algorithm
can be re-distributed to various epochs
so that the computation cost
associated with any {level-$\ell$ epoch}
 is bounded by $O(5^{\ell})$, for any $\ell \ge 0$.
%Moreover, the computation cost associated with any level-0 epoch is 0.
\end{lemma}
%\vspace{-3pt}
\begin{proof}
%The rest of this section is devoted to the proof of Lemma \ref{basiccost}.  % which is inherently different from arguments in \cite{BGS11}.
%[[S: maybe add a begin and end proof. Also, need to say something about the general proof outline]]
%To cover that cost, the basic idea is to show that
%It is deferred to App.\ \ref{redist} due to space constraints. %complicates things up.
%Formally, we will show that the total number of epochs created
%and terminated
%throughout the update sequence
%is small with respect to the total costs associated with them.
%When charging a certain computation cost to the creation cost (resp., termination cost) of some epoch, we essentially ``charge the future'' (resp., ``charge the past'');
%i.e., this charging is based on future (resp., past) edge deletions from the graph that are expected to occur.
%We will show that, in this sense, the costs of Procedure $\detr$ (resp., Procedure $\rand$)  charge the past (resp., future).
%. More concretely, if the matched edge is $(u,v)$ and $u$
%is the vertex initiating the epoch's creation, then $v$ is chosen as $u$'s mate by the algorithm uniformly at random among at least $5^{\ell}$ neighbors of $u$.
%Using this fact, we will be able to reason that each epoch
%[[S: maybe should outline the general goal, where the cost of any epoch should be exponential in its level.
%Also, for an epoch at level $\ell$, we must show that the mate was chosen uniformly at random among $5^{\ell-1}$ optional mates.
%\footnote{[[S: The reason I use $\ell-1$ rather than $\ell$ in the superscript is because level-1 epochs are handled deterministically, so we have just 1 optional mate.
%On the other hand, maybe this could help improving the leading constant (by a factor of 3); if not, we can always define the level of free vertices to be -1,
%and the level of deterministically matched vertices to be 0]]}
%Summarizing, we have proved the following lemma.  % is an immediate corollary of the charging scheme.   %follows easily from the charging argument given above.
The update algorithm is triggered following edge insertions and edge deletions.
Following an edge insertion, we apply
%\paragraph{Edge insertion.}
Procedure $\ins(u,v)$. This procedure is called at most once per update step, and its runtime is constant.
We may disregard this constant cost (formally, we charge this cost to the corresponding update step).
Hence, the lemma holds vacuously for edge insertions.

Following an edge deletion, we apply
Procedure $\del(u,v)$. This procedure is called at most once per update step; disregarding the calls to $\evalf(u)$ and $\evalf(v)$, this procedure's runtime is constant.
We henceforth disregard this constant cost (charging it to the corresponding update step), and demonstrate how to re-distribute the costs of the calls to $\evalf(u)$ and $\evalf(v)$ to
appropriate epochs in a manner satisfying the condition of the lemma.

Let $z \in \{u,v\}$. The execution of Procedure $\evalf(z)$ splits into two cases.
In the first case $\dout(z) < 5^{\ell_z+1}$, and Procedure $\evalf(z)$ invokes Procedure $\detr(z)$, whose runtime is $O(5^{\ell_z})$.
Even though Procedure $\detr(z)$ may create a new level-0 epoch, there is no need to charge this epoch with any costs.
% aiming again to guarantee that level-0 epochs will have zero costs.
The entire cost $O(5^{\ell_z})$ of Procedure $\detr(z)$ is charged to the termination cost of epoch $\cE((u,v),l)$ (triggered by the deletion of edge $(u,v)$ from the graph).
 which is of level $\ell_z$, thus satisfying the condition of the lemma.

Otherwise $\dout(z) \ge 5^{\ell_z+1}$, and Procedure $\evalf(z)$ calls $\rand(z)$.

The runtime of Procedure $\rand(z)$ may be much larger than $5^{\ell_z}$ and even than $\dout(z)$.
To cover the costs of this procedure, we create a new epoch at a sufficiently high level, attempting to charge the costs of the procedure to the creation cost of the new epoch.
However, this charging attempt may sometimes fail, in which case we call the procedure recursively.
Each recursive call will create a new epoch at yet a higher level,  attempting to charge the yet-uncharged costs of
the procedure to the creation cost of the most recently created epoch.
Since the levels of epochs created during this process grow by at least one  with each recursion level, this recursive process will terminate.
Specifically, the depth of this recursive process is bounded by $\log_5 (n-1)$.
(Formally, one should also take into account the calls to Procedure $\evalf$ from within Procedure $\rand$, which may, in turn, invoke Procedure $\rand$.\footnote{Since the assertion
that the recursive process terminates is a corollary of our ultimate bound on the update time,
an additional proof is not required. Nevertheless, a simpler proof
that is  independent of our proof of the update time bound is sketched in the full version \cite{Solom16}.})
\ignore{
 %over all vertices $v$ in the graph.
We define a  \emph{potential function} $f(G) = \sum_{v \in V} {5^{\ell_v}}$ for the dynamic graph $G$ with respect to the dynamic level assignment of its vertices.
The initial call to Procedure $\rand$ may trigger a single call to Procedure $\evalf$.
Each subsequent recursive call to Procedure $\rand$ may trigger two calls to Procedure $\evalf$.
It can be easily verified that each call to Procedure $\rand$ must increase the potential by at lease one unit more than the calls to Procedure $\evalf$ that it triggers may decrease it.
Each such call to   $\evalf$ may, in turn, invoke Procedure $\rand$.
Nevertheless, the potential growth due to each such call to Procedure $\rand$ is at least 1,
regardless of whether it is a recursive call invoked by Procedure $\rand$ itself
or a new call invoked by Procedure $\evalf$.
Since the potential value is upper bounded by $n \cdot 5^{\log_5(n-1)} \le n^{2}$ at all times, it follows that the total number of calls to Procedure $\rand$
is   upper bounded by $n^2$; in particular, this number is finite, thus the recursive process must terminate.
}
%charging argument, which proves that the amortized update time of the algorithm is constant.)
Next, we describe the charging argument in detail.

%
For each recursion level of Procedure $\rand$,
our charging argument may (slightly) \emph{over-charge} the current level's costs,
so as to cover some of the yet-uncharged costs incurred by  previous recursion levels.
%which may be as high as $O(5^{\ell^*})$,
%in addition to
Denote by $\rand(z^{(i)})$ the $i$th recursive call, with $z^{(i)}$ being the examined vertex.
The initial call to Procedure $\rand$ may be viewed as the 0th recursion level.  %, and has no additional costs.
As argued below (see Claim \ref{conc}), it may leave a ``debt''
%of $O(5^{\ell_z})$ units of cost (where $\ell_z$ is the out-degree of the examined vertex),
%which does not exceed $O(5^{\ell^*})$ by definition, but may be of the same order of magnitude.
%As a result,
to the 1st recursion level, but this debt must be bounded by $O(\dout(z^{(1)}))$ units of cost.
In general, for each $i \ge 1$, the \emph{debt} at recursion level $i$ (left by previous recursion levels) must be bounded by  $O(\dout(z^{(i)}))$;
in what follows we may view this debt as part of the costs incurred at level $i$. (Note that the initial call to the procedure has no debt.)

Observe that the $i$th recursive call $\rand(z^{(i)})$ may also invoke Procedure $\evalf$.
Our charging argument views the call to   $\evalf$ as part of the execution of $\rand(z^{(i)})$.
More concretely, the costs incurred by the call to $\evalf$ are charged to epochs that are created or terminated throughout the execution of the $i$th recursive call $\rand(z^{(i)})$.
Note, however, that Procedure $\evalf$ may, in turn, invoke Procedure $\rand$.
Our charging argument does \emph{not} view the new call to $\rand$ as part of the execution of $\rand(z^{(i)})$, but rather as an \emph{independent} call.
More concretely, the costs of the new call to Procedure $\rand$ are
%independent of the costs of the original call, and they are
charged only to epochs that are created or terminated throughout the execution of this new call to   $\rand$.

% may start with this ``debt'',
%which should be able to cover it, in addition to its own cost.

%The following claim completes the charging argument, thus 
To conclude the proof of Lemma \ref{basiccost}, we use the following claim, whose proof
%is omitted due to space constraints, but appears in
is deferred to the full version \cite{Solom16}.
\begin{claim} \label{conc}
%(We may define $z = z^{(0)}$.)
For any $i \ge 0$, we can re-distribute the costs of the $i$th recursive call $\rand(z^{(i)})$ of Procedure $\rand$ (including the debt from previous recursion levels, if any)
to various epochs, allowing a potential debt to the subsequent recursive call $\rand(z^{(i+1)})$ (if the procedure proceeds to recursion level $i+1$),
so that:
\vspace{2pt}\\(1) The cost charged to any level-$\ell$ epoch is bounded by $O(5^{\ell})$, for any $\ell$. 
\vspace{2pt}\\(2) The debt left for recursion level $i+1$ is bounded by $O(\dout(z^{(i+1)}))$.
If the procedure terminates at recursion level $i$, then no debt is allowed, i.e., the entire cost in this case is re-distributed to the epochs.
%The debt at recursion level $i$ (left by previous recursion levels) is  $O(\dout(z^{(i)}))$, for $i \ge 1$.
%(2) An epoch may be charged with costs only if they are directly related to one of its endpoints.
\end{claim}
\ignore{
\begin{proof}
The proof is by induction on the recursion level $i$.
Recall that the initial call $\rand(z^{(0)})$ of the procedure, which corresponds to the basis $i=0$ of the induction, has no debt.
Nevertheless, the basis of the induction and the induction step are handled together as follows.

Consider the $i$th recursive call $\rand(z)$, $i \ge 0$, writing $z = z^{(i)}$ to avoid cluttered notation.
Observe that the debt from previous recursion levels is bounded by $O(\dout(z))$ units of cost.
(This observation follows from the induction hypothesis for $i-1$, unless $i=0$, in which case it holds vacuously.)
To cover this debt, the procedure creates a new epoch of sufficiently high level,
determined as the minimum level $\ell^* = {\ell^*}^{(i)}$ after $\ell_z$ such that $\phi_z(\ell^*+1) < 5^{\ell^*+1}$.
By Lemma \ref{rand_basic}(4), computing this level $\ell^*$ requires $O(5^{\ell^*})$ time, which, by Lemma \ref{rand_basic}(3),
already supersedes the debt of $O(\dout(z))$ units of cost from previous recursion levels; we may henceforth disregard this debt.
%Even though this step by itself can be implemented more efficiently, there is no need for efficiency here. Indeed, ==
% namely, of
%If the debt is of value $O(5^{\ell
%level $\ell^*$ defined as above.
The procedure then sets the level of $z$ to $\ell^*$ by calling to $\setlvl(z,\ell^*)$.
%which involves flipping all incoming edges from vertices of level at most $\ell^* -1$ to be outgoing of $v$.
By Lemma \ref{rand_basic}(4), the runtime of this call is $O(5^{\ell^*})$.
Then a random outgoing neighbor $w$ of $z$  is chosen as a mate for $z$,
% $S_{\ell^* - 1}$ of all neighbors of $z$ with level at most $\ell^*-1$, from which a vertex $w$ is chosen uniformly at random as a mate for $z$,
and its level is set to $\ell^*$ by calling to $\setlvl(w,\ell^*)$.
%We are guaranteed that the cost of the call to $\setlvl(z,\ell^*)$ is bounded by $O(d_{\ell^*}(z)) = O(5^{\ell^*})$. However,
By Observation \ref{ob:setlevel}(3), the runtime of this call is $O(\dout(w) + \ell^*)$, where $\dout(w)$ is $w$'s new out-degree, and it may be that $\dout(w) \gg 5^{\ell^*}$.
%.  %The execution of the procedure splits into two cases.
In the case that $\dout(w) < 5^{\ell^*+1}$, disregarding a potential call to $\evalf(w')$ that is addressed below,
the entire cost of the $i$th recursive call  $\rand(z^{(i)})$  of the procedure is $O(5^{\ell^*})$, and we charge it to the creation cost of the new  level-$\ell^*$ epoch $\cE((z,w),l)$.
In this case the procedure terminates at recursion level $i$, and no debt whatsoever is left.
%This charging satisfies all the conditions of the lemma, and completes the induction step in this case.

If $\dout(w) \ge 5^{\ell^*+1}$, Procedure $\rand(z)$ deletes the new matched edge $(z,w)$ from the matching, thus terminating the respective epoch
$\cE((z,w),l)$.
Then it proceeds to recursion level $i+1$  by making a recursive call to $\rand(w)$,  with $w = z^{(i+1)}$.
By Lemma \ref{rand_basic}(1), this recursive call is guaranteed to create a new epoch at level $\ell'$ higher than $\ell^*$.
Moreover, Lemma \ref{rand_basic}(3) implies that $\dout(w) < 5^{\ell' + 1}$,
%it can be charged with cost at least $\Omega(\dout(w))$.
and so the cost $O(\dout(w) + \ell^*) = O(\dout(w)) = O(5^{\ell'})$ of the call to $\setlvl(w,\ell^*)$ made in the $i$th recursion level can be charged to the creation cost of the  new level-$\ell'$ epoch
that is created in recursion level $i+1$.
Concretely, we ``drag'' the cost of the call to $\setlvl(w,\ell^*)$, which is the aforementioned debt, to the $(i+1)$th recursion level.
Observe that this debt does not exceed the out-degree of the examined vertex $w = z^{(i+1)}$ by more than a constant factor, as required.  %the condition of the induction step holds.
%Indeed, in the recursive call $\rand(w)$, we will have a debt of cost $\dout(w)$.
%[[S: need to explain that the level is guaranteed to be greater than $\ell^*$ and at least (check???) logarithmic in the new out-degree.]]
%The remaining parts of Procedure $\rand(z)$ boil down to calls t
%NEED TO SAY STUFF ABOUT E.G.

%There is also a potential call to $\evalf(z)$. Recall that we charged $O(5^{\ell_z})$ of the costs of the original call to $\evalf(z)$ to
%the termination cost of epoch $\cE((u,v),l)$ (triggered by the deletion of edge $(u,v)$ from the graph).
%Similarly, we charge $O(5^{\ell^*})$ of the costs of the current call to $\evalf(z)$ to the termination cost of the new epoch $\cE((z,w),l)$.
%If the current call's costs exceed $O(5^{\ell^*})$, they will also be charged to newly created epochs following the scheme described above.
%We stress that   the creation and termination costs of the level-$\ell^*$ epoch $\cE((z,w),l)$ are both bounded by $O(5^{\ell^*})$, as required.
There is also a potential call to $\evalf(z)$; recall that $z$ is a shortcut for $z^{(i)}$.
This call should not be confused with the original call to $\evalf(z)$, in which case $z$ is used as a shortcut for $z^{(0)}$.
In what follows we abandon these shortcuts, and write either $z^{(0)}$ or $z^{(i)}$ explicitly, to avoid ambiguity.
Moreover, this call should not be confused with the $i$th recursion call to the procedure, which we currently analyze.
Recall that we charged $O(5^{\ell_{z^{(0)}}})$ units of cost out of the costs of the original call to $\evalf(z^{(0)})$ to
the termination cost of epoch $\cE((u,v),l)$ (triggered by the deletion of edge $(u,v)$ from the graph).
Similarly, we charge $O(5^{\ell^*})$ units of cost out of the costs of the new call to $\evalf(z^{(i)})$ to the termination cost of the level-$\ell^*$ epoch $\cE((z^{(i)},w),l)$
(triggered by the deletion of edge $(z^{(i)},w)$ from the matching).
%If the costs of the current call to $\evalf(z)$ exceed $O(5^{\ell^*})$, they will also be charged to newly created epochs following the scheme described above.
Observe that the only way for the costs of $\evalf(z^{(i)})$ to exceed
$O(5^{\ell^*})$ is due to a call to $\rand(z^{(i)})$. (Indeed, if a call to $\detr(z^{(i)})$ is made, then its cost is bounded by $O(\dout(z^{(i)})) = O(5^{\ell^*})$.)
Moreover, the new call to   $\rand(z^{(i)})$
%be confused with either the original call $\rand(z^{(0)})$
%or the $i$th recursion call analyzed above, but should rather
is analyzed independently of the original call $\rand(z^{(0)})$ and the $i$th recursion call to the procedure currently analyzed.
%both these calls.
In particular,   the costs of the new call to $\rand(z^{(i)})$
%are not viewed as part of the costs of both these calls,
%and
are charged only to epochs that are created or terminated as part of this new call, and should not be taken into account in this induction proof.
%the new call to Procedure $\rand$.
%not viewed as part of the costs of $\rand(z^{(i)})$. Indeed,
%There is also a potential call to $\evalf(w')$, whose cost is charged to the termination cost of epoch $\cE((w,w'),l)$,
%unless it exceeds $O(5^{\ell_{w'}})$, in which case it will also be charged to newly created epochs.

Finally, there is   a potential call to $\evalf(w')$.
We charge $O(5^{\ell_{w'}})$ units of cost out of the costs of this call to the termination cost of the level-$\ell_{w'}$ epoch $\cE((w,w'),l)$
(triggered by the deletion of edge $(w,w')$ from the matching).
Similarly to above, the only way for the costs of $\evalf(w')$ to exceed $O(5^{\ell_{w'}})$ is due to a call to $\rand(w')$.
%in which case they will also be charged to newly created epochs following the above scheme.
The costs of the call to $\rand(w')$, however, are
%not viewed as part of the costs of the original call to Procedure $\rand$,
charged only to epochs that are created or terminated as part of this new call to Procedure $\rand$,  and should not be taken into account in this induction proof.
%costs are not viewed as part of the costs of $\rand(z^{(i)})$.
%Formally, the calls to $\evalf(\cdot)$ from within the $i$th call of the procedure are not charged.

Summarizing, the costs of the $i$th recursion call $\rand(z^{(i)})$ are re-distributed to epochs subject to the requirements of the claim:
%in a manner satisfying the conditions of the claim.
(i) At most $O(5^{\ell^*})$ units of cost are charged to  the creation and termination costs of the level-$\ell^*$ epoch $\cE((z^{(i)},w),l)$.
(ii) At most $O(5^{\ell_{w'}})$ units of cost are charged to the termination cost of the level-$\ell_{w'}$ epoch $\cE((w,w'),l)$.
% are both bounded by $O(5^{\ell^*})$, as required.
%If $w$ was previously matched to $w'$, then the epoch $\cE((w,w'),t)$ is terminated.
% but we do not charge the termination cost anything.
(iii) The debt left for recursion level $i+1$ (if the procedure proceeds to that level) is bounded by $O(\dout(z^{(i+1)}))$.
The induction step follows.
%In general, this charging scheme does not let any level-$\ell$ epoch ``absorb''
%as much of the computation cost taking place on its endpoints  as possible, but never
%let a level-$\ell$ epoch absorb
%more than $O(5^{\ell})$ units of cost.
\end{proof}
}
\vspace{3pt}
By Claim \ref{conc}, whenever Procedure $\rand$  terminates, no debt whatsoever is left.
Consequently, the entire cost of this procedure (over all recursion levels) can be re-distributed to various epochs
in a manner satisfying the conditions of  Lemma \ref{basiccost}.
%This completes the proof of
 Lemma \ref{basiccost} follows.
\end{proof}
%[[S: Here is a good place to sketch the intuition of everything (in particular, we use the info on incoming neighbors)]]
%[[S: must distinguish between level-0 epochs and epochs of higher levels. Need to explain that level-0 epochs are created via $\detr$
%and higher level epochs are created via $\rand$.]]
%[[S: right, the first assertion would not hold for level-0 epochs, but it does hold for higher levels. It is a direct corollary of Claim 2.1.
%May need to recall the dichotomy between level-0 epochs and those at higher levels]]
%In other words, This enables us to charge this cost of $O(5^{\ell^*})$ to the creation cost of the new epoch, because in the amortized sense this epoch can cover
%an expected.
\vspace{7pt}
%\\
\noindent
{\bf 3.4~ Natural versus induced epochs.~}
An epoch corresponding to edge $(u,v)$ is terminated either because edge $(u,v)$ is deleted from the graph, and then it is called a \emph{natural epoch},
or because the update algorithm deleted edge $(u,v)$ from the matching, and then it is called an \emph{induced epoch}.
%By Corollary \ref{basiccost}, the cost of any level-0 epoch is 0.
Following \cite{BGS11}, we will charge the computation cost of each induced epoch $\cE$ of level $\ell \ge 0$ to the cost of the unique epoch $\cE'$ whose creation ``triggered'' the termination of
$\cE$.

An induced epoch is terminated only by Procedure $\rand$. Consider the first call to Procedure $\rand(z)$, which we also view as the 0th recursion level.
 %, and for exactly one of two reasons.
%\\\emph{Case 1:
First, some vertex $w$ of level $\ell_w$ lower than $\ell^*$ is chosen as a random mate for   vertex $z$, and a level-$\ell^*$ epoch $\cE((z,w),l)$ is created.
If $w$ is matched to $w'$, the edge $(w,w')$ is deleted from the matching, and we view the creation of the level-$\ell^*$ epoch $\cE((z,w),l)$ as terminating the
level-$\ell_{w'}$ epoch $\cE((w,w'),l)$.
Next, suppose that
%the out-degree of $w$ is ``too large'', i.e., if epoch $\cE((v,w),t)$ is of level $\ell^*$, then
$\dout(w) \ge 5^{\ell^*+1}$. In this case the newly created epoch $\cE((z,w),l)$
is terminated, and immediately afterwards we make the 1st recursive call to $\rand(w)$.
By Lemma \ref{rand_basic}(1), the call to $\rand(w)$ is guaranteed to create a new epoch $\cE((w,x),l)$ at level $\ell'$ higher than $\ell^*$,
where $x$ is a random outgoing neighbor of $w$, which is of level $\ell_x$ lower than $\ell'$ by Lemma \ref{rand_basic}(2).
We view the creation of the level-$\ell'$ epoch $\cE((w,x),l)$ as terminating the level-$\ell^*$ epoch $\cE((z,w),l)$. Furthermore, if $x$ is matched to $x'$, the edge $(x,x')$ is deleted from the matching,
and we view the creation of the level-$\ell'$ epoch $\cE((w,x),l)$ as terminating the level-$\ell_{x'}$  epoch $\cE((x,x'),l)$ as well.
%We have shown that the creation of epoch $\cE((v,w),l)$ terminates (at most) one epoch of lower level, whereas
We have shown that the creation of epoch $\cE((w,x),l)$ at the 1st recursion level terminates (at most) two epochs of lower levels.
%In this case, the creation of a single epoch is viewed as terminating two distinct epochs, whereas in the first reason it terminated just a single epoch.
%In this sense the second case subsumes the first case. More accurately,
Exactly the same reasoning applies to an arbitrary recursion level $i$ by induction.
%The first case corresponds to the 0th recursion level of Procedure $\rand$, where the creation of an epoch terminates just a single epoch.
%The second case corresponds to higher levels of recursion, and
%However, then the creation of a single epoch may terminate two distinct epochs.
To summarize, the creation of a new epoch terminates at most two epochs, both of which are of levels
%Furthermore, the levels of the terminated epochs are 
strictly lower than that of the created epoch.
%both of level at most $\ell - 1$. The first impression is that the creation of a new epoch may cause only a single epoch to terminate.
%Indeed, whenever some vertex $v$ chooses uniformly at random a vertex $w$ in $S^{\ell^*-1}$ as its mate, the only epoch that may terminate is $\cE((w,w'),t)$,
%assuming $w$ was not free. However, this situation reflects well just the first level of the recursion of Procedure $\rand(v)$.
%Consider the next recursive call $\rand(w)$, which matches the vertex $w$ with some new random vertex, say $x$.
%Of course, if $x$ was previously matched to some vertex $x'$, then the termination of epoch $\cE((x,x'),t)$ is inevitable.
%However, before proceeding recursively, the epoch corresponding to edge $(v,w)$ must be terminated.
That is, if the level of the created epoch is $\ell$ and the levels of the terminated epochs are $\ell_1$ and $\ell_2$,
then $\ell_1,\ell_2 < \ell$.

We say that a level $\ell$  is \emph{induced}
%our assumption does not hold, i.e.,  $T_\ell > 2X_\ell$,
%We claim that such levels can be disregarded from the runtime analysis.
%whence
if the number of induced level-$\ell$ epochs  
%at level $\ell$
exceeds the number of natural level-$\ell$ epochs; otherwise it is \emph{natural}.
Next, we show that the computation costs incurred by any induced level can be charged to the computation costs at higher levels.
%allowing us to disregard any level where the assumption does not hold in the runtime analysis.
% at that level.
%As $T_\ell > 2X_\ell$,
Specifically, in any induced level $\ell$ we can define a one-to-one mapping from the natural to the induced epochs.
%mapping each natural level-$\ell$ epoch to a unique induced level-$\ell$ epoch.
For each induced epoch, at most one natural epoch (at the same level) is mapped to it; any natural epoch that is mapped to an induced epoch is called \emph{semi-natural}.
By definition, for any induced level $\ell$, all natural $\ell$-level epochs are semi-natural.  % under this definition.
For the natural levels, however, we do not define such a mapping.
Thus for any natural level, all natural epochs terminated at that level remain as before; these epochs are called \emph{fully-natural}.

%Then we can (temporarily) charge the costs of any level-$\ell$ natural epoch to the induced epoch to which it is mapped
%In Section 4.3, we defined the recursive cost of an epoch as the sum of its actual cost and the recursive costs of the at most two induced
%epochs (at lower levels) terminated by it. Let us re-define the recursive cost of an epoch
%as the sum of its actual cost and the recursive costs of the at most two induced epochs terminated by it as well as the at most two natural epochs
%corresponding to them under the aforementioned mapping.

%We henceforth change the constant 3 to 5 throughout the paper; in particular, instead of using $\log_5(n-1)$ levels, we will use $\log_5(n-1)$ levels.
%Consequently, we allow the computation cost associated with any level-$\ell$ epoch to grow from $O(5^\ell)$ to  $O(5^\ell)$ (cf.\ Lemma \ref{basiccost}),
%and obtain the recurrence $\hat C_{\ell} \le   4 \hat C_{\ell-1} + O(5^{\ell})$,
%with the base condition
%$\hat C_{0} =  O(1)$, which resolves to $\hat C_{\ell} = O(5^{\ell})$ (cf.\ Corollary \ref{important}).
%???
%???

We  define the \emph{recursive cost} of an epoch as the sum of its actual cost and the recursive costs of the (at most) two induced epochs terminated by it
as well as the (at most) two semi-natural epochs mapped to them; the recursive cost of a level-0 epoch is its actual cost.
%[[S: maybe we shouldn't attempt to bound the cost of a 0-level epoch by 0; constant should also do. The recurrence will resolve to something slightly larger, but it will
%save a few lines before]]
Denote the highest   recursive cost of any level-$\ell$ epoch by $\hat C_\ell$, for any $\ell \ge 0$. (Obviously $\hat C_\ell$ is monotone non-decreasing with $\ell$.)
By Lemma \ref{basiccost}, we get the recurrence $\hat C_{\ell} \le  \hat 2C_{\ell_1} +  2\hat C_{\ell_2} + O(5^{\ell}) \le  4 \hat C_{\ell-1} + O(5^{\ell})$,
where $\ell_1,\ell_2 < \ell$,
with the base condition
$\hat C_{0} =  O(1)$. This recurrence resolves to $\hat C_{\ell} = O(5^{\ell})$.

%\vspace{-2.5pt}
\begin{corollary} \label{important}
For any $\ell \ge 0$, the recursive cost of any level-$\ell$ epoch is bounded by $O(5^{\ell})$.
\end{corollary}
%\vspace{-2pt}

By definition, the sum of recursive costs over all fully-natural epochs is equal to the sum of actual costs over all  epochs (fully-natural, semi-natural and induced)
that have been \emph{terminated} throughout the update sequence.
\vspace{7pt}
\\
\noindent
{\bf 3.5~ Bounding the algorithm's runtime.~}
During any sequence of $t$ updates, the total number of epochs created equals the number of epochs terminated and the number of epochs
that \emph{remain alive} at the end of the $t$ updates.
To bound the computation cost charged to all epochs that remain alive at the end of the update sequence,
one may use an argument similar to \cite{BGS11}.
However, instead of distinguishing between terminated epochs and ones that remain alive,
we find it cleaner to get rid of those epochs that remain alive by deleting all edges of the final graph, one after another.
That is, we append  additional edge deletions at the end of the original update sequence, so as to finish with an empty graph.
The order in which these edges are deleted from the graph may be random, but it may also be deterministic,
as long as it is oblivious to the maintained matching.
 %e.g., it can be determined deterministically according to some lexicographic rules that are fixed at the outset of the algorithm.
% or according to by a random order.

This tweak guarantees that no epoch remains alive at the end of the update sequence.
As a result, the sum of recursive costs over all fully-natural epochs will bound the sum of actual costs over all  epochs (fully-natural, semi-natural and induced)
that have been \emph{created} (and also terminated) throughout the update sequence, or in other words, it will bound the total runtime of the algorithm.
Note that the total runtime of the algorithm may only increase as a result of this tweak.
Since we increase the length of the update sequence by at most a factor of 2,
an amortized runtime bound of the algorithm with respect to the new update sequence will imply the same (up to a factor of 2) amortized bound with respect to the original sequence.

\ignore{
consider a level-$\ell$ epoch  corresponding to edge $(u,v)$ that belongs to the matching at the end of the $t$ update steps, and suppose that $u$ initiated the creation of this epoch
at update step $l$.
By Corollary \ref{important}, the recursive cost charged to that epoch is $O(5^\ell)$.
By Corollary \ref{Ob:basic}(1), if $\cO^l_u$ is the set of $u$'s outgoing neighbors at step $l$,
then $|\cO^l_u| \ge 5^\ell$. Note also that $|\cO^l_u| \le t_u$, where $t_u$ is the number of edge updates ever incident on $u$.
Since any vertex may be part of at most one epoch that is alive at the end of the update sequence, the total computation cost charged to all such epochs
is bounded by $\sum_{u \in V} O(t_u) = O(t)$.
}

%In order to bound this sum,
%To bound this quantity,
%, with the main hurdle being the high probability bound.
% cost of all natural epochs.
%$c \cdot 5^{\ell} (1 + 2/3 + 4/9 + ...$.
%[[S: specify the leading constants]]
%\begin{remark}
%Notice that the recurrence $\hat C_{\ell} = 2\hat C_{\ell-1} + O(2^\ell)$, with the same base condition, resolves to $O(2^\ell \cdot \ell)$.
%This is the reason we used the constant 3 rather than 2 as in \cite{BGS11}. However, in fact, there is no reason to use a different constant.
%To see this, note that...
%\end{remark}
%[[S: remove this remark]]
%Suppose that the epoch corresponds to edge $(v,w)$, and that it is initiated by vertex $v$.
%\vspace{7pt}
%\\
%\noindent{\bf 4.4~ Bounding the sum of recursive costs over all natural epochs.~}
%\label{sec:cost}
%In this section
%We follow the argument of \cite{BGS11} to analyze the number of natural epochs that are terminated throughout the entire update sequence,
%and then strengthen this argument in order to derive stronger high probability bounds.
% and Lemma \ref{expect}, the sum of recursive costs over all natural epochs
%terminated at level $\ell$ is $O(t_\ell)$ in expectation and $O(t_\ell + \log n \cdot 5^\ell)$ w.h.p.
%Hence,
%the sum of recursive costs over all natural epochs terminated
%during the entire sequence is $\sum_{\ell \ge 0} O(t_\ell) = O(t)$ in expectation and $\sum_{\ell \ge 0} O(t_\ell + \log n \cdot 5^\ell) = O(t + n \log n)$ w.h.p.
Let $Y$  be the r.v.\ for the sum of recursive costs over all fully-natural epochs terminated during the entire sequence.
Note that $Y$ stands for the total runtime of the algorithm.  %'s total runtime.
%this is due to the fact that Lemma \ref{expect} builds on
%and appear in Appendix \ref{app:prob} for completeness.
%\vspace{-12pt}
\begin{lemma}  \label{expect}
%(1) $\Expect(Y) = O(t)$. (2)
$Y = O(t + n \log n)$ w.h.p.
\end{lemma}  
The proof of Lemma \ref{expect} is deferred to the full version \cite{Solom16}.
While it follows similar lines as in \cite{BGS11}, the bound   it provides shaves a logarithmic factor from the bound of \cite{BGS11}.
(This is because our algorithm is inherently different than the BGS algorithm and since other parts in the analysis are different.)
Moreover, there is a significant difference between our proof and that of BGS.
In particular, we extend the epoch definition as follows.
Consider an arbitrary epoch initiated by some vertex $u$ at some update step $l$.
%and let $\cO^{l}_{u}$ denote the set of $u$'s outgoing neighbors at that time.
An epoch is terminated when its matched edge $(u,v)$ becomes unmatched (i.e., deleted from the matching);
the \emph{(interrupted) duration of the epoch} is defined as the number of outgoing edges of $u$ at time $l$
that get deleted  from the graph between time step $l$ and the epoch's termination.
This definition of duration is given in \cite{BGS11}, and it coincides with the epoch definition of Section 3.2.
%(All these edge deletions occur at level $\ell$ by definition.)
We define the \emph{uninterrupted duration} of the epoch as the number of outgoing edges of $u$ at time $l$
that get deleted from the graph between time step $l$ and the time that the random matched edge $(u,v)$ is deleted \emph{from the graph}.
%(Since we appended edge deletions at the end of the original update sequence to guarantee that the final graph is empty,
%all the outgoing edges of $u$ at time $l$, including edge $(u,v)$, will get deleted throughout the update sequence.)

Roughly speaking, to prove Lemma \ref{expect}, one should establish independence between the durations of the various epochs,
and then employ it to argue that sufficiently many epochs at each level have w.h.p.\ long durations.  % and argue that many of the epochs have long durations,
To this end, we find it crucial to analyze the uninterrupted durations of epochs rather than their (interrupted) durations.
If the epoch is natural, its uninterrupted duration equals its duration. For an induced epoch, however,
its uninterrupted duration 
%On the negative side, the uninterrupted duration of an induced epoch
may be significantly larger than its duration.  %, which poses a nontrivial challenge:
Consequently, proving that many epochs at each level have w.h.p.\ long \emph{uninterrupted} durations is rather useless, if it turns out that most of them are induced.
For this reason, we need to be able to restrict our attention to levels where there are sufficiently many natural epochs,
and this is exactly why we distinguished between natural and induced levels, or analogously, between fully-natural and semi-natural epochs.
%(Note also that the outgoing edges of $u$ at time $l$ that get deleted from the graph after the epoch's termination are not necessarily deleted at level $\ell$.)

%and is given mainly for completeness
It is not difficult to extend the high probability proof to obtain $\Expect(Y) = O(t + n \log n)$.
%\vspace{2pt}
%\begin{lemma} [Proof in Appendix \ref{app:prob}]  \label{prob}
%$X_i$ is $O(t_i / 5^i + \log n)$ with high probability.
%\end{lemma}
%\subsection{Wrapping up} \label{sec:wrap}
Shaving the $O(n \log n)$ term from the high probability bound, and consequently from the expected bound, requires additional new ideas; 
see the full version \cite{Solom16} for the details.
We remark that there are alternative   proofs for obtaining an expected bound of $O(t)$, without deriving it from the high probability bound.
%(Such a proof was communicated to us by Sayan Bhattacharya, Manoj Gupta, Divya
%\subsubsection
%Thus, at least $\dout^{new}(v) - \sqrt{t} \ge 2\sqrt{t}$ of $v$'s outgoing neighbors have level strictly lower than $\ell_{max}(t)$.
%Procedure $\rand(v)$ simply% have level strictly lower than $\ell_{max}(t)$.
%and we choose a mate for $v$ uniformly at random out of $\Theta(\sqrt{t})$ of them within $O(\sqrt{t})$ time.
%Consequently, the level of $v$ will remain the same, and the corresponding epoch is chosen at an appropriate probability.
%Wait a second. In the worst-case we have a redundant term of $\log n \cdot 2^j$ from each $j = 1,2,\ldots,\approx \log (n^{3/4})$,
%so we get a slack of at most $n^{3/4} \log n$, and that's nothing...


Finally, the space usage of our algorithm is linear in the dynamic number of edges in the graph.
%(In Baswana et al.'s algorithm \cite{BGS11}, to maintain the $\phi_v(\cdot)$ values, an array of logarithmic size is maintained for each vertex $v$, hence the space usage is %$\Omega(n \log n)$.) Summarizing, we have proved:
%To summarize, one can maintain maximal matching with constant update time and linear space.
%\vspace{-1pt}
\begin{theorem}
Starting from an empty graph on $n$ fixed vertices, a maximal matching (and thus 2-MCM and also 2-MCVC) can be maintained over any sequence of $t$ edge insertions and deletions
in $O(t)$ time in expectation and w.h.p., and using $O(n+m)$ space, where $m$ denotes the dynamic number of edges.
%For any update sequence of length $t$ that start from an empty graph, there is a randomized algorithm for maintaining a maximal matching within total expected time $O(t)$.
%The time bound holds with high probability, and the space usage of the algorithm is
%$O(n +m)$, where $n$ is the fixed number of vertices and $m$ is the constantly changing number of edges.
\end{theorem}



%\section{Linear Space}
%[[S: don't forget, my $d_\ell(v)$ is the same as their $\phi_\ell(v)$, the only difference is that they tried to minimize the max index $\ell$ whereas I try to minimize it.
%Change my notation to be in accordance to theirs]]
\ignore{
\section{Discussion and Open Questions}
I suggest to say that it would be interesting to obtain worst-case bounds, and that we believe that our ideas can lead to $2+\eps$-MCM
with roughly the same update time $O(f(\eps))$, but we don't know how to achieve optimality.
It's also reasonable not to have this section, so that it seems that everything is closed
}
%\clearpage
%\ignore{
\vspace{7pt}
%\noindent
{\bf Acknowledgements.~}
The author is grateful to Amir Abboud, Surender Baswana, Sayan Bhattacharya, Manoj Gupta, David Peleg, Sandeep Sen, Noam Solomon  and Virginia Vassilevska Williams for helpful discussions.
%}
\ignore{
\section*{Acknowledgements}
The author thanks Amir Abboud, David Peleg and Virginia Vassilevska Williams for helpful discussions.
%[[S: maybe say as above (grateful, timely...). run spell checker. go over Sections 2 and 3]]
}
%\clearpage

%[[S: don't forget to add papers on matchings by Kapralov and Pettie and other PC members]]

%\bibliographystyle{latex8}
%\bibliography{randomMMbibfile}
\begin{thebibliography}{1}  %\setlength{\itemsep}{1.463ex}\small

\bibitem{AW14}
A.~Abboud and V.~V. Williams.
\newblock Popular conjectures imply strong lower bounds for dynamic problems.
\newblock In {\em Proc. 55th FOCS}, pages 434--443, 2014.

\bibitem{ABGS12}
A.~Anand, S.~Baswana, M.~Gupta, and S.~Sen.
\newblock Maintaining approximate maximum weighted matching in fully dynamic
  graphs.
\newblock In {\em Proc. 32nd FSTTCS}, pages 257--266, 2012.

\bibitem{BGS11}
S.~Baswana, M.~Gupta, and S.~Sen.
\newblock Fully dynamic maximal matching in ${O}(\log n)$ update time.
\newblock In {\em Proc. of 52nd FOCS}, pages 383--392, 2011.

\bibitem{BS15}
A.~Bernstein and C.~Stein.
\newblock Fully dynamic matching in bipartite graphs.
\newblock In {\em 42nd ICALP}, pages 167--179, 2015.

\bibitem{BS16}
A.~Bernstein and C.~Stein.
\newblock Faster fully dynamic matchings with small approximation ratios.
\newblock In {\em Proc. of 26th SODA}, pages 692--711, 2016.

\bibitem{BHI15}
S.~Bhattacharya, M.~Henzinger, and G.~F. Italiano.
\newblock Deterministic fully dynamic data structures for vertex cover and
  matching.
\newblock In {\em Proc. 26th SODA}, pages 785--804, 2015.

\bibitem{CW77b}
L.~Carter and M.~N. Wegman.
\newblock Universal classes of hash functions.
\newblock In {\em Proc. 9th STOC}, pages 106--112, 1977.

\bibitem{DP14}
R.~Duan and S.~Pettie.
\newblock Linear-time approximation for maximum weight matching.
\newblock {\em J. {ACM}}, 61(1):1, 2014.

\bibitem{Gupta14}
M.~Gupta.
\newblock Maintaining approximate maximum matching in an incremental bipartite
  graph in polylogarithmic update time.
\newblock In {\em Proc. 34th FSTTCS}, pages 227--239, 2014.

\bibitem{GP13}
M.~Gupta and R.~Peng.
\newblock Fully dynamic $(1+\epsilon)$-approximate matchings.
\newblock In {\em 54th FOCS}, pages 548--557, 2013.

%\bibitem{GS09}
%M.~Gupta and A.~Sharma.
%\newblock An $o(\log(n))$ fully dynamic algorithm for maximum matching in a
%  tree.
%\newblock {\em CoRR}, abs/0901.2900, 2009.

\bibitem{HTZ14}
M.~He, G.~Tang, and N.~Zeh.
\newblock Orienting dynamic graphs, with applications to maximal matchings and
  adjacency queries.
\newblock In {\em Proc. 25th ISAAC}, pages 128--140, 2014.

\bibitem{HK73}
J.~E. Hopcroft and R.~M. Karp.
\newblock An n$^{\mbox{5/2}}$ algorithm for maximum matchings in bipartite
  graphs.
\newblock {\em SIAM J. Comput.}, 2(4):225--231, 1973.

\bibitem{IL93}
Z.~Ivkovi\'{c} and E.~L. Lloyd.
\newblock Fully dynamic maintenance of vertex cover.
\newblock In {\em 19th WG}, pages 99--111, 1993.

\bibitem{KKM13}
B.~M. Kapron, V.~King, and B.~Mountjoy.
\newblock Dynamic graph connectivity in polylogarithmic worst case time.
\newblock In {\em Proc. of 24th SODA}, pages 1131--1142, 2013.

\bibitem{KR08}
S.~Khot and O.~Regev.
\newblock Vertex cover might be hard to approximate to within 2-epsilon.
\newblock {\em J. Comput. Syst. Sci.}, 74(3):335--349, 2008.

\bibitem{KKPS14}
T.~Kopelowitz, R.~Krauthgamer, E.~Porat, and S.~Solomon.
\newblock Orienting fully dynamic graphs with worst-case time bounds.
\newblock In {\em Proc. 41st ICALP}, pages 532--543, 2014.

\bibitem{KPP16}
T.~Kopelowitz, S.~Pettie, and E.~Porat.
\newblock Higher lower bounds from the {3SUM} conjecture.
\newblock In {\em Proc. of 26th SODA}, pages 1272--1287, 2016.

\bibitem{LPP08}
Z.~Lotker, B.~Patt{-}Shamir, and S.~Pettie.
\newblock Improved distributed approximate matching.
\newblock In {\em Proc.  SPAA}, pages 129--136, 2008.

\bibitem{LPR09}
Z.~Lotker, B.~Patt{-}Shamir, and A.~Ros{\'{e}}n.
\newblock Distributed approximate matching.
\newblock {\em {SIAM} J. Comput.}, 39(2):445--460, 2009.

\bibitem{MV80}
S.~Micali and V.~V. Vazirani.
\newblock An ${O}(\sqrt{|{V}|} |{E}|)$ algorithm for finding maximum matching
  in general graphs.
\newblock In {\em Proc. 21st FOCS}, pages 17--27, 1980.

\bibitem{NS13}
O.~Neiman and S.~Solomon.
\newblock Simple deterministic algorithms for fully dynamic maximal matching.
\newblock In {\em Proc. 45th STOC}, pages 745--754, 2013.

\bibitem{OR10}
K.~Onak and R.~Rubinfeld.
\newblock Maintaining a large matching and a small vertex cover.
\newblock In {\em Proc.  STOC}, pages 457--464, 2010.

\bibitem{PelB00}
D.~Peleg.
\newblock {\em Distributed Computing: A Locality-Sensitive Approach}.
\newblock SIAM, 2000.

\bibitem{PS16}
D.~Peleg and S.~Solomon.
\newblock Dynamic $(1 + \epsilon)$-approximate matchings: A density-sensitive
  approach.
\newblock In {\em Proc. of 26th SODA}, pages 712--729, 2016.

%\bibitem{Pettie12}
%S.~Pettie.
%\newblock A simple reduction from maximum weight matching to maximum
%  cardinality matching.
%\newblock {\em Inf. Process. Lett.}, 112(23):893--898, 2012.

\bibitem{Sank07}
P.~Sankowski.
\newblock Faster dynamic matchings and vertex connectivity.
\newblock In {\em Proc. 18th SODA}, pages 118--126, 2007.

\bibitem{Solom16}
S.~Solomon.
\newblock Fully Dynamic Maximal Matching in Constant Update Time.
\newblock {\em CoRR}, abs/1604.08491, 2016.

\bibitem{Vaz12}
V.~V. Vazirani.
\newblock An improved definition of blossoms and a simpler proof of the {MV}
  matching algorithm.
\newblock {\em CoRR}, abs/1210.4594, 2012.

\end{thebibliography}

%\clearpage

\ignore{
\clearpage
\pagenumbering{roman}
\appendix
\centerline{\LARGE\bf Appendix}

%\vspace{-10pt}
\section{Tables and Pseudocode} \label{app:tab}
%\vspace{-10pt}

\begin{table*}[thb]
\begin{center}
\resizebox {\textwidth }{!}{
\footnotesize
\begin{tabular}{|c||c|c|c|}
\hline Reference & Update time   & Space & Bound  \\
\hline
\hline
The na\"{\i}ve algorithm & $O(n)$ & $O(n+m)$ & deterministic \\
\hline
Ivkovi\'{c} and Lloyd (WG'93) \cite{IL93} & $O((n+m)^{\frac{\sqrt{2}}{2}})$ & " & " \\
\hline
Neiman and Solomon (STOC'13) \cite{NS13}  & $O(\sqrt{m})$ & " & "    \\
%\hline
%\hline
%Gupta and Sharma \cite{GS09}  (MCM in trees) & $O(\log n)$ & " & " \\
%  & & & \\
\hline
\hline
Neiman and Solomon (STOC'13) \cite{NS13}  & $O(\inf_{\beta > 1}(\alpha \beta +\log_{\beta}n))$ & " & "    \\
for $\alpha = O(1)$ & $O(\log n/ \log\log n)$ & " & " \\
%\hline Kopelowitz et al.\ (ICALP'14) \cite{KKPS14} & $O(\inf_{\beta > 1}\{\alpha^2 \beta^2 + \alpha \beta \lceil \log_\beta n \rceil\})$  & " & "  \\
%for $\alpha = O(1)$   &  $O(\log n)$ & " & "   \\
\hline He et al.\ (ISAAC'14) \cite{HTZ14} &  $O(\alpha + \sqrt{\alpha \log n})$ & " & "   \\
 for $\alpha = O(1)$   &  $O(\sqrt{\log n})$ & " & "   \\
\hline
\hline Baswana et al. (FOCS'11) \cite{BGS11} &   $O(\log n)$ & $O(n \log n + m)$ & expected    \\
    " &    $O(\log n + (n \log^2 n)/t)$ & " & w.h.p.\    \\
\hline
\hline {\bf  This paper} &   {\boldmath $O(1)$} & {\boldmath $O(n+m)$} & {\bf expected and w.h.p.}  \\
\hline
\end{tabular}
}
\end{center}
\vspace{-0.1in}
\caption[]{ \label{tab1} \footnotesize A   comparison of   previous and our results
for dynamic maximal matchings.
The parameter $t$ (used for describing the result of \cite{BGS11}) designates the total number of updates
and the parameter $\alpha$ (used for describing the results of \cite{NS13,HTZ14}) designates the \emph{arboricity}
bound of the dynamic graph, i.e., it is assumed that the dynamic graph has arboricity at most $\alpha$ at all times.
(The \emph{arboricity} $\alpha(G)$ of a graph $G$ is the minimum number of edge-disjoint forests into which it can be partitioned,
and it is close to the density of its densest subgraph; for any $m$-edge graph, its arboricity ranges between 1 and $\sqrt{m}$.)
}
\end{table*}



\begin{table*}[thb]
\begin{center}
\resizebox {\textwidth }{!}{
\footnotesize
\begin{tabular}{|c||c|c|c|}
\hline Reference & Approximation & Update time   & Bound  \\
\hline
\hline Bhattacharya et al.\ (SODA'15)   \cite{BHI15} & $3+\eps$ & $O(\min\{\sqrt{n}/\eps,m^{1/3}\cdot \eps^{-2}\})$ & deterministic  \\
\hline Bernstein and Stein (SODA'16)   \cite{BS16} & $3/2+\eps$ & $O(m^{1/4} \cdot \eps^{-2.5})$ & " \\
\hline
Neiman and Solomon (STOC'13) \cite{NS13}  & $3/2$ & $O(\sqrt{m})$ & "    \\
\hline Gupta and Peng (FOCS'13) \cite{GP13}  & $1+\eps$ & $O(\sqrt{m} \cdot \eps^{-2})$ &  "   \\
\hline
\hline Gupta and Sharma \cite{GS09} (for trees) & 1 & $O(\log n)$ & " \\
\hline
%\hline {\bf  This paper} & {\boldmath $1+\eps$} & {\boldmath  & {\bf \cmark}  \\
\hline Bernstein and Stein (SODA'16)  \cite{BS16} & $3/2+\eps$ & $O(\alpha(\alpha + \log n + \eps^{-2}) + \eps^{-6})$ & "  \\
\hline Peleg and Solomon (SODA'16) \cite{PS16} & $3/2+\eps$ & $O(\alpha/\eps)$ & " \\
\hline Bernstein and Stein (ICALP'15)  \cite{BS15} & $1+\eps$ & $O(\alpha(\alpha + \log n) + $ & "  \\
(bipartite graphs of bounded arboricity) & &  $\eps^{-4}(\alpha + \log n) + \eps^{-6})$ & \\
\hline Peleg and Solomon (SODA'16) \cite{PS16} & $1+\eps$ & $O(\alpha \cdot \eps^{-2})$ & " \\
%     for $\alpha = O(1), \eps = O(1)$ & " & $O(\log n)$ & " \\
\hline
\hline Neiman and Solomon (STOC'13) \cite{NS13}  & 2 & $O(\inf_{\beta > 1}(\alpha \beta +\log_{\beta}n))$ & "    \\
%\hline Kopelowitz et al.\ (ICALP'14) \cite{KKPS14} & " & $O(\inf_{\beta > 1}\{\alpha^2 \beta^2 + \alpha \beta \lceil \log_\beta n \rceil\})$  & "  \\
\hline He et al.\ (ISAAC'14) \cite{KKPS14} & " &  $O(\alpha + \sqrt{\alpha \log n})$ & "  \\
\hline
\hline Onak and Rubinfeld \cite{OR10} & $c$ & $O(\log^2 n)$ & w.h.p. \\
\hline Baswana et al. (FOCS'11) \cite{BGS11} & 2  &   $O(\log n)$ & expected  \\
    " & "  & $O(\log n + (n \log^2 n)/t)$ &  w.h.p. \\
\hline
\hline {\bf  This paper} & {\boldmath $2$} & {\boldmath $O(1)$} & {\bf expected and w.h.p.} \\
%{\bf  for} {\boldmath $\alpha = O(1), \eps = O(1)$}  & " & {\boldmath $O(1)$} & " \\
%\hline {\bf  This paper} & {\boldmath $3/2+\eps$} & {\boldmath $O(\alpha/\eps)$} & {\bf \cmark} \\
%  {\bf  for} {\boldmath $\alpha = O(1), \eps = O(1)$} & {\boldmath "} & {\boldmath $O(1)$} & {\bf "}  \\
%\hline {\bf  This paper} & {\boldmath $1+\eps$} & {\boldmath $O(\alpha \cdot \eps^{-2})$} & {\bf \cmark}  \\
% {\bf  for} {\boldmath $\alpha = O(1), \eps = O(1)$} & {\boldmath "} & {\boldmath $O(1)$} & {\bf "}  \\
\hline
\end{tabular}
}
\end{center}
\vspace{-0.1in}
\caption[]{ \label{tab2} \footnotesize A comparison of previous and our results
for dynamic approximate MCMs. The parameter $t$ designates the total number of updates,
$\alpha$ designates the arboricity bound of the dynamic graph and $c$ is a sufficiently large constant.
In contrast to all other results, the matching maintained in \cite{GS09} is not represented \emph{explicitly}: In order to determine if an edge belongs to the matching, one should run an $O(\log n)$-time query. This result appears in the table for completeness.
%As mentioned above, in contrast to all other results, the matching maintained in \cite{GS09} is not represented explicitly.
}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[thb]
\begin{center}
\resizebox {\textwidth }{!}{
\footnotesize
\begin{tabular}{|c||c|c|c|}
\hline Reference & Approximation & Update time   & Bound  \\
\hline \hline
%Cohen \cite{Coh93} & $(2k-1)\cdot(1+\eps)$ &
Neiman and Solomon (STOC'13) \cite{NS13}  & $2$ & $O(\sqrt{m})$ & deterministic   \\
%\hline Kopelowitz et al.\ (ICALP'14) \cite{KKPS14} & 2 & fixed arboricity & \cmark & \cmark & \xmark \\
\hline
\hline Neiman and Solomon (STOC'13) \cite{NS13}  & 2 & $O(\inf_{\beta > 1}(\alpha \beta +\log_{\beta}n))$ & "  \\
%\hline Kopelowitz et al.\ (ICALP'14) \cite{KKPS14} & 2 & $O(\inf_{\beta > 1}\{\alpha^2 \beta^2 + \alpha \beta \lceil \log_\beta n \rceil\})$  & "  \\
\hline He et al.\ (ISAAC'14) \cite{KKPS14} & 2 &  $O(\alpha + \sqrt{\alpha \log n})$ & "  \\
  \hline
\hline Bhattacharya et al.\ (SODA'15)   \cite{BHI15} & $2+\eps$ & $O(\log n \cdot \eps^{-2}\})$ & " \\
\hline
\hline Peleg and Solomon (SODA'16) \cite{PS16} &   $2+\eps$ & $O(\alpha/\eps)$ & "  \\
  \hline
  \hline Onak and Rubinfeld \cite{OR10} & $c$ & $O(\log^2 n)$ & w.h.p. \\
  \hline Baswana et al. (FOCS'11) \cite{BGS11} & 2  & expected $O(\log n)$ & expected  \\
    " & " & $O(\log n + (n \log^2 n)/t)$ & w.h.p.  \\
    \hline
\hline {\bf  This paper} & {\boldmath $2$} & {\boldmath $O(1)$} & {\bf expected and w.h.p.} \\
\hline
\end{tabular}
}
\end{center}
\vspace{-0.1in}
\caption[]{ \label{tab3} \footnotesize A  comparison of previous and our results for dynamic approximate MCVCs.
The parameter $t$ designates the total number of updates,
$\alpha$ designates the arboricity bound of the dynamic graph and $c$ is a sufficiently large constant.
%The parameter $\alpha$ designates the arboricity bound of the dynamic graph, $t$ designates the total number of updates
%and $c$ is a sufficiently large constant.
}
\end{table*}

%\vspace{-13pt}

\begin{figure}[!ht]
\fbox{
\begin{minipage}[t]{165mm}
$\ins(u,v)$:
\begin{enumerate}\itemsep1.5pt \parskip2pt \parsep2pt
\item $N_v \leftarrow N_v \cup \{u\}$;
\item $N_u \leftarrow N_u \cup \{v\}$;
\item If $\ell_u \ge \ell_v$:
 /* orient the edge from $u$ to $v$ */
   \begin{enumerate}\itemsep1.5pt \parskip2pt \parsep2pt
   \item $\cO_u \leftarrow \cO_u \cup \{v\}$;
   \item $\cI_v[\ell_u] \leftarrow \cI_v[\ell_u] \cup \{u\}$;
   \end{enumerate}
\item Else:
 /* orient the edge from $v$ to $u$ */
   \begin{enumerate}\itemsep1.5pt \parskip2pt \parsep2pt
   \item $\cO_v \leftarrow \cO_v \cup \{u\}$;
   \item $\cI_u[\ell_v] \leftarrow \cI_u[\ell_v] \cup \{v\}$;
   \end{enumerate}
\item If $\ell_u = \ell_v = -1$:  /* if $u$ and $v$ are free, match them */
%\mate(u) = \mate(v) = \bot$:
   \begin{enumerate}\itemsep1.5pt \parskip2pt \parsep2pt
   \item  $M \leftarrow M \cup \{(u,v)\}$;
   \item $\setlvl(u,0)$;
   \item $\setlvl(v,0)$;
   \end{enumerate}
\end{enumerate}
\end{minipage}}
\caption{Handling edge insertion $(u,v)$.
}
\label{fig:handleIns}
\end{figure}

\begin{figure}[!ht]
\fbox{
\begin{minipage}[t]{165mm}
$\del(u,v)$:
\begin{enumerate}\itemsep2pt \parskip2pt \parsep2pt
\item $N_v \leftarrow N_v \setminus \{u\}$;
\item $N_u \leftarrow N_u \setminus \{v\}$;
\item If $v \in \cO_u$:
 /* if edge $(u,v)$ is oriented from $u$ to $v$ */
   \begin{enumerate}\itemsep2pt \parskip2pt \parsep2pt
   \item $\cO_u \leftarrow \cO_u \setminus \{v\}$;
   \item $\cI_v[\ell_u] \leftarrow \cI_v[\ell_u] \setminus \{u\}$;
   \end{enumerate}
\item Else:
   \begin{enumerate}\itemsep2pt \parskip2pt \parsep2pt
   \item $\cO_v \leftarrow \cO_v \setminus \{u\}$;
   \item $\cI_u[\ell_v] \leftarrow \cI_u[\ell_v] \setminus \{v\}$;
   \end{enumerate}
\item If $(u,v) \in M$:
 /* delete edge $(u,v)$ from the matching */
   \begin{enumerate}\itemsep2pt \parskip2pt \parsep2pt
   \item  $M \leftarrow M \setminus \{(u,v)\}$; /* $u$ and $v$ become temporarily free, their levels exceed -1 */
   \item $\evalf(u)$;
   \item $\evalf(v)$;
   \end{enumerate}
\end{enumerate}
\end{minipage}}
\caption{Handling edge deletion $(u,v)$.
}
\label{fig:handleDel}
\end{figure}

\begin{figure}[!ht]
\fbox{
\begin{minipage}[t]{165mm}
$\setlvl(v,\ell)$:
\begin{enumerate}\itemsep2pt \parskip2pt \parsep2pt
    \item For all $w \in \cO_v$:  /* update $\cI_w$ regarding $v$'s new level  */
       \begin{enumerate}\itemsep2pt \parskip2pt \parsep2pt
        \item $\cI_w[\ell_v] \leftarrow \cI_w[\ell_v] \setminus \{v\}$;
        \item $\cI_w[\ell] \leftarrow \cI_w[\ell] \cup \{v\}$;
        \end{enumerate}

\item If $\ell < \ell_v$: /* in this case the level of $v$ is decreased by at least one */
    \begin{enumerate}\itemsep2pt \parskip2pt \parsep2pt
    \item For all $w \in \cO_v$ such that $\ell+1 \le \ell_w \le \ell_v$:
     /* flip $v$'s outgoing edge $(v,w)$ */
       \begin{enumerate}\itemsep2pt \parskip2pt \parsep2pt
        \item $\cO_v \leftarrow \cO_v \setminus \{w\}$;
        \item $\cI_v[\ell_w] \leftarrow \cI_v[\ell_w] \cup \{w\}$;
        \item $\cI_w[\ell] \leftarrow \cI_w[\ell] \setminus \{v\}$;
        \item $\cO_w \leftarrow \cO_w \cup \{v\}$;
        \end{enumerate}
   \end{enumerate}

\item If $\ell > \ell_v$: /* in this case the level of $v$ is increased by at least one */
 \begin{enumerate}\itemsep2pt \parskip2pt \parsep2pt
%    \item For all $w \in \cI_v[i]$ with $\ell_v \le i \le \ell-1$:
    \item For all $i = \ell_v,\ldots,\ell-1$ and all $w \in \cI_v[i]$:
    %/* scan $\cI_v$ sequentially until passing level $\ell-1$ */
   /* flip $v$'s incoming edge $(v,w)$ */
%     \begin{enumerate}
%     \item
       \begin{enumerate}\itemsep2pt \parskip2pt \parsep2pt
       \item $\cI_v[i] \leftarrow \cI_v[i] \setminus \{w\}$;
       \item $\cO_v \leftarrow \cO_v \cup \{w\}$;
       \item $\cO_w \leftarrow \cO_w \setminus \{v\}$;
       \item $\cI_w[\ell] \leftarrow \cI_w[\ell] \cup \{v\}$;
       \end{enumerate}
   % \end{enumerate}
\end{enumerate}
\item  $\ell_v \leftarrow \ell$;
\end{enumerate}
\end{minipage}}
\caption{Setting the old level $\ell_v$ of $v$ to   $\ell$.}
\label{fig:setlvl}
\end{figure}

\begin{figure}[!ht]
\fbox{
\begin{minipage}[t]{165mm}
$\evalf(v)$:
\begin{enumerate}\itemsep2pt \parskip2pt \parsep2pt
\item If $\dout(v)  < 5^{\ell_v+1}$: $\detr(v)$;
\item Else $\rand(v)$;
\end{enumerate}
\end{minipage}}
\caption{Handling a vertex that becomes temporarily free.
}
\label{fig:evalfree}
\end{figure}

\begin{figure}[!ht]
\fbox{
\begin{minipage}[t]{165mm}
$\detr(v)$:
\begin{enumerate}\itemsep2pt \parskip2pt \parsep2pt
\item For all $w \in \cO_v$:
       \begin{enumerate}\itemsep2pt \parskip2pt \parsep2pt
        \item If $\ell_w = -1$: /* if $w$ is free, match $v$ with $w$ */
        \begin{enumerate}\itemsep2pt \parskip2pt \parsep2pt
        \item  $M \leftarrow M \cup \{(v,w)\}$;
        \item $\setlvl(v,0)$;
        \item $\setlvl(w,0)$;
        \item terminate;
        \end{enumerate}
   \end{enumerate}
 \item \setlvl(v,-1); /* all  outgoing neighbors of $v$ are matched, hence $v$ becomes free */
\end{enumerate}
\end{minipage}}
\caption{Matching $v$ with a free neighbor  (if exists) deterministically. %in which case a matching edge $(v,w)$ at level 0 is created.
It is assumed that $\dout(v)  < 5^{\ell_v+1}$.
}
\label{fig:detr}
\end{figure}

\begin{figure}[!ht]
\fbox{
\begin{minipage}[t]{165mm}
$\rand(v)$:
\begin{enumerate}\itemsep2pt \parskip2pt \parsep2pt
\item $\ell^* \leftarrow \ell_v$;
\item while $\phi_v(\ell^*+1) \ge 5^{\ell^*+1}$: $\ell^* \leftarrow \ell^* + 1$;
%\begin{enumerate}
%\end{enumerate}
\\ /* $\ell^*$ is the minimum level after $\ell_v$ with $\phi_v(\ell^*+1) < 5^{\ell^*+1}$ */
\item $\setlvl(v,\ell^*)$; /* after this call $\ell_v = \ell^*$ and $5^{\ell^*} \le \dout(v) = \phi_v(\ell^*) < 5^{\ell^* + 1}$ */
%\\ /* moreover, $v$'s outgoing neighbors are its neighbors of level lower than $\ell^*$ */

%\item Let $S_{\ell^* - 1}$ contain all vertices in $\cO_v$ and all vertices in $\cI_v[i]$, for $\ell_v \le i \le \ell^* - 1$.
%\\ /* $S_{\ell^* - 1}$ contains all neighbors of $v$ of level at most $\ell-1$ */
%\\ /* note that $5^{\ell^*} < |S_{\ell^*-1}| = d_{\ell^*-1}(v)  \le 5^{\ell^*+1}$ */
\item Pick an outgoing neighbor $w$ of $v$ uniformly at random;
\\ /* $w$ is chosen with probability at most $1/5^{\ell^*}$ and $\ell_w \le \ell^* -1$ */
\item $w' \leftarrow \mate(w)$;
\item If $w' \ne \bot$: $M \leftarrow M \setminus \{(w,w')\}$;
\item $\setlvl(w,\ell^*)$; /* in order to match $v$ to $w$, they need to be at the same level */
\item $M \leftarrow M \cup \{(v,w)\}$;
%\item for $w \in \cO_v$:
%       \begin{enumerate}
%        \item If $\ell_w = 0$: /* equivalent to checking if $w$ is free */
%        \begin{enumerate}
\item If $\dout(w) \ge  5^{\ell^*+1}$:
    \begin{enumerate}\itemsep2pt \parskip2pt \parsep2pt
    \item $M \leftarrow M \setminus \{(v,w)\}$; /* after this command is executed, $\mate(v) = \mate(w) = \bot$ */
    \item $\rand(w)$; /* before this call, $\dout(w) \ge  5^{\ell^*+1} = 5^{\ell_w+1}$ */
    \item If $\mate(v) = \bot$: $\evalf(v)$; /* if $v$ is temporarily free, handle it */
    \end{enumerate}
\item If $w' \ne \bot$ and $\mate(w') = \bot$: $\evalf(w')$; /* if $w'$ is temporarily free, handle it */
%        \end{enumerate}
  % \end{enumerate}
\end{enumerate}
\end{minipage}}
\caption{Matching $v$ at level $\ell^*$ higher than $\ell_v$, with a random neighbor $w$ of level lower than $\ell^*$.
%The procedure attempts to add such a matching edge $(v,w)$ at level $\ell^*$
If this   requires too much time, the procedure calls itself recursively to match $w$ at yet a higher level, in which case $v$ becomes free and handled via Procedure $\evalf(v)$.
It is assumed that $\dout(v)  \ge 5^{\ell_v+1}$.
}
\label{fig:rand}
\end{figure}

%\section{Description of Procedure $\setlvl(v,\ell)$} \label{setlevel}

\ignore{
\section{Some More Details on the Data Structures} \label{app:data}
%It is important that the hash table $\cI_v$ is sorted according to the level of its elements,
%so that $\cI_v[\ell]$ will come before $\cI_v[\ell']$ in that list if $\ell < \ell'$.
While the number of pointers stored in the  dynamic hash table $\cI_v$ is bounded by $\log_5 (n-1)+2$, it may be much smaller than that.
%Since there are no incoming neighbors of level 0, there is no need to consider level $-1$.
%$\cA_v[0]$ points to an empty list
Indeed, there is no pointer in $\cI_v$ corresponding to level smaller than $\ell_v$,
implying that the number of pointers stored in $\cI_v$ is at most $\log_5 (n-1) + 1 -\ell_v$.
Note also that no incoming neighbor of $v$ is of level -1 (by Invariant \ref{exception}), thus there is no pointer in $\cI_v$ corresponding to level -1.
Recall that pointers to empty lists are not stored in the hash table, thus the total space over all hash tables is at most linear in the dynamic number of edges
in the graph. If we were to store the pointers in a static array, then the total space over these arrays would be $\Omega(n \log n)$.
In the case that the dynamic graph is usually dense (i.e., having $\Omega(n \log n)$ edges), it is advantageous to use arrays,
as it is easier to implement all the basic operations (delete, insert, search), and the time bounds become deterministic.

%
%
%The hash table (or array) $\cI_v$ is also suitably augmented with a linked list storing the pointers of $\cI_v$, so that for any parameter $\ell \ge \ell_v$,
%we can retrieve all pointers of $\cI_v$ between levels $\ell$ and $\ell_v$ in time linear in their number.
%
%
%While the data structure $\cI_v$ provides information on the levels of $v$'s incoming neighbors,

Note that no information whatsoever on the levels of $v$'s outgoing neighbors is provided by the data structure $\cO_v$.
In particular, to determine if $v$ has an outgoing neighbor at a certain level (most importantly at level -1, i.e., a free neighbor),
we need to scan the entire list $\cO_v$. On the other hand, $v$ has an incoming neighbor at a certain level $\ell$ iff
the corresponding list $\cI_v[\ell]$ is non-empty.
It will not be in $v$'s \emph{responsibility} to maintain the
%$\cO_v$,
%whereas maintaining the
data structure $\cI_v$, but rather within the responsibility of $v$'s incoming neighbors.


As mentioned, we keep mutual pointers between the elements in the various data structures: For any vertex $v$ and any outgoing neighbor $u$ of $v$,
we have mutual pointers between all elements $u \in \cO_v, v \in \cI_u[\ell_v],v \in N_u,u \in N_v$.
%Whenever an edge $(u,v)$ is inserted to the graph and oriented as ${\orient u v}$, we add elements $v$ and $u$ to $N_u$ and $N_v$, respectively
For example, when  an edge $(u,v)$ oriented as ${\orient v u}$ is deleted from the graph,
we get a pointer  to either $v \in N_u$ or $u \in N_v$, and through this pointer we delete all elements $u \in \cO_v, v \in \cI_u[\ell_v],v \in N_u,u \in N_v$.
As another example, when  the orientation of edge $(u,v)$ is flipped from ${\orient u v}$ to ${\orient v u}$, then assuming we have
a pointer to   $v \in \cO_u$ (which is   the case in our algorithms), we can reach element $u \in \cI_v[\ell_u]$ through the pointer, delete them both from the respective lists,
and then create elements $u \in \cO_v$ and $v \in \cI_u[\ell_v]$ with mutual pointers.
We also keep mutual pointers between a matched edge  and its endpoints.
%We do not address
(We do not provide a complete description of the straightforward yet tedious maintenance of these pointers for the sake of brevity.)
%(The straightforward yet tedious maintenance of these pointers is not presented in more detail for obvious reasons.)
%We stress that our update algorithm never has to access \emph{specific} neighbors of some vertex via these pointers \emph{directly},
%but rather
%, and they never access elements of those lists \emph{directly}
%without these pointers.
%Therefore, there is no need to use sophisticated data structures for maintaining the outgoing and incoming neighbors of a vertex.
}
%the $i$th cell $\cA_v[i]$ points to an empty list, for each index $0 \le i \le \max\{0,\ell_v-1\}$.

%\section{Proof of Lemma \ref{basiccost}} \label{redist}

%\vspace{-13pt}
\section{Proof  of Lemma \ref{expect}} \label{app:prob}

While both endpoints of a matched edge are of the same level, this may not be the case for an unmatched edge.
We say that an edge $e$ is \emph{deleted at level} $\ell$ (from the graph) if \emph{at least one} of its endpoints is at level $\ell$
at the time of the deletion.
(Thus each edge is deleted at either one or two levels.
While the same edge can be deleted and inserted multiple times in an update sequence, we view different occurrences of the same edge as different objects.)
Let $S_\ell$ denote the sequence of edge deletions at level $\ell$,   write $|S_\ell| = t_\ell$, and denote by $t_{del}$ the total number of deletions;
Note that $t_\ell$ is a random variable (r.v.).
Then $\sum_{\ell \ge 0} t_\ell \le 2t_{del} \le t$.
Let $T_\ell = T_\ell(S_\ell)$ be the r.v.\ for the total number of epochs (fully-natural, semi-natural and indcued) terminated at level $\ell$.  %, and assume that $T_\ell \le 2X_\ell$;
%in Section \ref{justify} we demonstrate that this assumption does not lose generality.
(Since we made sure that the final graph is empty, any created epoch will get terminated throughout the update sequence.
Consequently, $T_\ell$ designates the total number of epochs created at level $\ell$ and $\sum_{\ell \ge 0} T_\ell$ designates the total number of epochs created
over all levels throughout the entire update sequence.)
Also, let $X_\ell = X_\ell(S_\ell)$ be the r.v. for the number of fully-natural epochs terminated at level $\ell$ for the update sequence $S_\ell$,
and let $Y_\ell$ be the r.v.\ for the sum of recursive costs over these epochs.
By Corollary \ref{important}, $Y_{\ell} = O(5^\ell) \cdot X_\ell$. (By definition, no epoch of any induced level $\ell$ is fully-natural, and so $X_\ell  = Y_\ell = 0$.)
%and thus $Y_\ell = 0$.)
Recall that $Y$ is the r.v.\ for the sum of recursive costs over all fully-natural epochs terminated during the entire sequence.
Thus we have $Y = \sum_{\ell \ge 0} Y_\ell$.  %all natural epochs terminated at level $\ell$.



%from Section \ref{sec:mainanal}
Fix an arbitrary level $\ell, 0 \le \ell \le \log_5 (n-1)$.
Consider any level-$\ell$ epoch initiated by some vertex $u$ at some update step $l$,
and let $\cO^{l}_{u}$ denote the set of $u$'s outgoing neighbors at that time.
By Corollary \ref{Ob:basic}, $|\cO^{l}_{u}| \ge 5^\ell$,
%$5^{\ell} \le |\cO^{l}_{u}| \le 5^{\ell+1}$,
and the mate $v$ of $u$ is chosen uniformly at random among all vertices of  $\cO^l_u$.
The epoch is terminated when the matched edge $(u,v)$ gets deleted \emph{from the graph};
recall that the \emph{(interrupted) duration of the epoch} is the number of outgoing edges of $u$ at time $l$
that get deleted  from the graph between time step $l$ and the epoch's termination.
(All these edge deletions occur at level $\ell$ by definition.)
Recall also that  the \emph{uninterrupted duration} of an epoch is the number of outgoing edges of $u$ at time $l$
that get deleted from the graph between time step $l$ and the time that the random matched edge $(u,v)$ is deleted from the graph.
(Since we appended edge deletions at the end of the original update sequence to guarantee that the final graph is empty,
all the outgoing edges of $u$ at time $l$, including edge $(u,v)$, will get deleted throughout the update sequence.)
Note that the outgoing edges of $u$ at time $l$ that get deleted from the graph after the epoch's termination are not necessarily deleted at level $\ell$.

For a natural epoch, its uninterrupted duration equals its duration. However, for an induced epoch,
its uninterrupted duration may be significantly larger than its duration.
Both notions of duration (interrupted and uninterrupted) are needed for the probabilistic argument to work,
and each of them is useful for different purposes.
The following observation shows that not too many epochs may have large (interrupted) duration.
(A similar statement cannot be made with respect to the uninterrupted duration.)
%Indeed, this is the natural motivation for using this notion of duration.
\begin{observation} \label{obs:duration}
If there are $q$   level-$\ell$ epochs with durations at least $\delta$,
then $q \le 2t_\ell / \delta$.
\end{observation}
\begin{proof}
Consider the edge deletions that define the durations of these $q$ epochs.
Any such edge deletion $(u,v)$ is associated with at most two epochs, one initiated by $u$ and possibly another one initiated by the other endpoint $v$.
Hence the total number of such deletions is bounded by $2t_\ell$, and we are done.
\end{proof}

\ignore{
\vspace{2pt}
\noindent
\\
%\subsection
{\bf Proof of   Lemma \ref{expect}(1):}~
We say that a level-$\ell$ epoch is \emph{short} if its duration is at most $(1/2) 5^{\ell}$;
%for some parameter $0 \le \mu \le 1$.
%A $1/2$-short epoch is also called \emph{short};
otherwise it is \emph{long}.
By definition, when a short epoch is terminated, at least half of the   edges among which the matched edge was randomly chosen   are still present in the graph.
Let $X^{short}_\ell$ and $X^{long}_\ell$ be the random variables for the number of short and long epochs terminated at level $\ell$, respectively.
By definition, we have $X_\ell = X^{short}_\ell + X^{long}_\ell$. By Observation \ref{obs:duration}, $X^{long}_\ell \le 2t_\ell / (5^{\ell}/2) = 4t_\ell / 5^\ell$.

%\begin{proof}
Let $e = (u,v)$ be an edge deleted (from the graph) at level $\ell$ during update step $l$, and let $Z_e$ be the indicator random variable
that takes value 1 if the deletion of edge $e$ causes termination of a \emph{short} epoch at level $\ell$, and 0 otherwise.
Observe that $X^{short}_\ell = \sum_{e \in S_\ell} Z_e$.
%Note that the number of long epochs terminated at level $\ell$ is bounded by $|S_\ell| / 5^\ell$.


Suppose that the deletion of edge $e$ causes termination of a short epoch at level $\ell$,
and assume w.l.o.g.\ that $u$ was the initiator of this epoch. Let $l'$ be the update step at which the corresponding epoch $\cE(e,l')$
was created, and let $\cO^{l'}_{u}$ be the set of $u$'s outgoing neighbors at that time.
By Corollary \ref{Ob:basic}, $|\cO^{l'}_{u}| \ge 5^\ell$.
Moreover, $u$ selects $v$ as its mate at update step $l'$ uniformly at random among all vertices of $\cO^{l'}_u$.
By Invariant \ref{exception}(c), the level of edge $e$ remains $\ell$ throughout the epoch's existence,
%In other words, the level of the two endpoints $u$ and $v$ remains $i$ during this entire time interval.
so if any of $u$'s outgoing edges at update step $l'$ is deleted during this time interval,  it is deleted at level $\ell$ by definition.
%It follows that any such edge deletion has the same probability of terminating the epoch as $e$ does.

We need to bound the probability  that the deletion of edge $e$ at update step $l$ causes termination of a short epoch at level $\ell$,
given that this epoch has not been terminated yet.
%the probability that the deletion of this edge causes termination of an epoch at level $\ell$, given that at most half of the $5^{\ell}$ outgoing
%edges of $u$ at time $l'$ have been deleted so far.
Since this epoch is short, it suffices to bound the probability that edge $e$ was chosen at step $l'$ among the at least $|\cO^{l'}_{u}|/2$
edges that are still present in the graph. We know that each of these edges has the same probability of being chosen, hence
this probability is bounded by $2/|\cO^{l'}_{u}|$,
%update step $l$
%Since any such edge deletion at level $i$ has the same probability of terminating the epoch as $e$ does,
and we have $\Prob(Z_e = 1) \le 2 / |\cO^{l'}_u| \le 2/5^\ell$.
Note also that $\sum_{\ell \ge 0} t_\ell \le t$, which implies that $\sum_{\ell \ge 0} \Expect(t_\ell) = \Expect(\sum_{\ell \ge 0} t_\ell) \le \Expect(t) = t$.
It follows that
\begin{eqnarray*}
\Expect(Y) &=& \sum_{\ell \ge 0} \Expect(Y_\ell) ~=~
\sum_{\ell \ge 0} O(5^{\ell}) \cdot \Expect(X_\ell) ~=~
\sum_{\ell \ge 0} O(5^{\ell}) \cdot (\Expect(X^{short}_\ell) + \Expect(X^{long}_\ell)) \\ &\le&
\sum_{\ell \ge 0} O(5^{\ell}) \cdot \left(\left(\sum_{e \in S_\ell} \Expect[Z_e] \right) + \Expect(X^{long}_\ell)\right)
~=~ \sum_{\ell \ge 0} O(5^{\ell}) \cdot \left(\left(\sum_{e \in S_\ell}  \Prob[Z_e = 1] \right) + (4/5^\ell) \Expect(t_\ell) \right)
\\  &\le& \sum_{\ell \ge 0} O(5^{\ell}) \cdot \left(\left(\sum_{e \in S_\ell} (2/5^\ell)\right) + (4/5^\ell) \Expect(t_\ell) \right)
~\le~ O(1) \cdot  \sum_{\ell \ge 0} \left(2t_\ell + 4\Expect(t_\ell)\right) ~=~  O(t). 
%\\ &=&  (3t_\ell / 5^{\ell})
\end{eqnarray*}
\ignore{

%\sum_{\ell \ge 0} O(t_\ell) = O(t)$.

By linearity of expectation,
$\Expect(X^{short}_\ell) ~=~ \sum_{e \in S_\ell} \Expect[Z_e] ~=~ \sum_{e \in S_\ell} \Prob[Z_e = 1] ~\le~ \sum_{e \in S_\ell} (2/5^\ell)$.
%2|S_\ell| / 5^\ell ~=~ 2t_\ell / 5^\ell.$
It follows that $$Y_\ell ~=~ O(5^{\ell}) \cdot X_\ell ~=~ O(5^{\ell}) \cdot (X^{short}_\ell + X^{long}_\ell) ~\le~  O(5^{\ell}) \cdot (3t_\ell / 5^{\ell})
~=~ O(t_\ell),$$ from which we conclude
}
%
%In other words, any of the outgoing edges of $u$ at update step $l'$
%\end{proof}
%\subsection
}
%\vspace{2pt}
%\noindent
%\\
%{\bf Proof of Lemma \ref{expect}(2):}~
%\begin{proof}
\ignore{
By Corollary \ref{Ob:basic}, $|\cO^{l}_{u}| \ge 5^\ell$,
and the mate $v$ of $u$ is chosen uniformly at random among all vertices of  $\cO^l_u$.
The epoch is terminated when the matched edge $(u,v)$ gets deleted (from the graph); we define the \emph{duration of the epoch} as the number of outgoing edges of $u$ at time $l$
that get deleted  between time step $l$ and the epoch's termination.
(All these edge deletions occur at level $\ell$ by definition.)
}



%Fix any level $\ell, 0 \le \ell \le \log_5 (n-1)$,
%consider a   level-$\ell$ epoch initiated by some vertex $u$ at some update step $l$,
%and let $\cO^{l}_{u}$ denote the set of $u$'s outgoing neighbors at that time.
The following observation shows that
%there cannot be too many epochs of large duration.
%We argue that the
an epoch's uninterrupted duration is a r.v.\ uniformly distributed in the range $[1,|\cO^l_u|]$.
This observation follows immediately from the fact that the matched edge is chosen uniformly at random among all the outgoing edges of $u$ at time $l$
and the fact that the adversary is oblivious to that choice.
(A similar statement cannot be made with respect to the interrupted duration.)
%a property which we will exploit in our probabilistic argument.
%This assertion would have been immediate if there were no induced epochs.
%Next, we demonstrate that the existence of induced epochs does not change the validity of the assertion.
\begin{observation} \label{eta}
For any $1 \le k \le |\cO^l_u|$, the probability that the uninterrupted duration of the epoch is
%epoch is natural and of duration
precisely $k$ equals $1 / |\cO^l_u|$.  % \le 1/5^\ell$.
%This bound remains valid even if it is given that the level of the epoch is $\ell$.
% and independently of epochs that were created previously to the current epoch.
 \end{observation}
 \ignore{
\begin{proof}
Denote the outgoing edges of $u$ at time $l$ by $e_1,e_2, \ldots, e_\rho$, where $\rho = |\cO^l_u|$,
let $d_1,d_2,\ldots,d_\rho$ denote the times at which these edges are deleted from the graph, respectively, and assume w.l.o.g.\ that $d_1 < d_2 < \ldots d_\rho$.
Denote the edge associated with the epoch by $e_i$.
%Assuming the epoch is natural,  it is terminated precisely at time $d_i$.
By time $d_i$, all edges $e_1,\ldots,e_{i}$ have been deleted from the graph,
but all edges $e_{i+1},\ldots,e_\rho$   remain there. Consequently, for the uninterrupted duration of the epoch to equal $k$, it must hold that $e_i = e_k$.
Thus the probability that the epoch's uninterrupted duration equals $k$ is given by the probability that its associated edge is $e_k$.
Since this edge is chosen uniformly at random among $\{e_1,\ldots,e_\rho\}$, the probability of choosing $e_k$ equals $1 / \rho = 1/ |\cO^l_u|$.
Moreover, this bound remains valid even if it is given that the epoch's level is $\ell$.
%then we argue that its associated edge must be $e_k$.
%Indeed, otherwise
\end{proof}
}
%Note that this claim implies that
%In other words, the epoch is $\mu$-short with probability at most $\mu$.

Note that the uninterrupted durations of distinct level-$\ell$ epochs are not necessarily independent.
In particular, the number $|\cO^l_u|$ of outgoing neighbors from which a mate $v$ for $u$ is chosen
may   well depend on previous coin flips of the algorithm. However, by Corollary \ref{Ob:basic},
%as the epoch is at level $i$,
it must be that $|\cO^l_u| \ge 5^\ell$.
%\item Second, although the mate of $u$ is chosen uniformly at random among all vertices in $\cO^l_u$,
%some of the optional choices may preclude future events from happening. Hence, future events may depend on this random choice.
%Moreover, this choice may well effect the (regular) durations of epochs that were created prior to it.
%However, this choice does not effect the uninterrupted durations of such epochs.  % in any way.
%Also, as $|\cO^l_u| \ge 5^\ell$, the probability that a specific vertex $v$ in $\cO^l_u$ is chosen as $u$'s random mate
%is bounded by $1/5^\ell$, independently of epochs that were created prior to the current epoch.
%it does not depend on the uninterrupted durations of previously created epochs in any way.  % in any way.
%\end{itemize}
Therefore, by Observation \ref{eta},
%Indeed, if $u$ and $u'$ are the vertices initiated these epochs, one at update step $l$ and the other at update step $l'$,
%then it is possible that the number $|\cO^l_u|$ of outgoing edges from which a mate $v$ for $u$ is chosen depends on
the probability that the uninterrupted duration of a level-$\ell$ epoch
 %is natural
%and of duration precisely
is precisely $k$ is bounded by $1/5^\ell$, for any $k$,
%due to the fact that the epoch is at level $i$,
%even if it is given that the level of the epoch is $\ell$, %, and more specifically,
independently of the uninterrupted durations of  epochs that were created prior to the current epoch.
%(Note that epochs that are created later on may depend on the current random choice.)  % made in the current epoch's creation.)
%E.g., maybe the fact that these epochs are at a certain level precludes some optional matched edges for the current epoch.)
A level-$\ell$ epoch is called \emph{$\mu$-short} if its \emph{uninterrupted} duration is at most $\mu \cdot 5^{\ell}$, for some parameter $0 \le \mu \le 1$.
We derive the following corollary.
%the epoch's duration is a random variable uniformly distributed in the range $[1,|\cO^l_u|]$.
%In particular,
\begin{corollary} \label{corborder}
For any $0 \le \mu \le 1$, the probability that an epoch is $\mu$-short is bounded by $\mu$,
%even if it is given that the level of the epoch is $\ell$, and
independently of the uninterrupted durations of epochs that were created prior to the current epoch's creation.
%its duration is at most $k$ with probability at most $k / |\cO^l_u| \le k/5^\ell$.)
\end{corollary}



%With a slight abuse of notation from the proof of the first assertion of this lemma,
%A $1/2$-short epoch is also called \emph{short}; otherwise it is \emph{long}.
%By definition, when a short epoch is terminated, at least half of the   edges among which the matched edge was randomly chosen   are still present in the graph.
%Let $X^{short}_\ell$ and $X^{long}_\ell$ be the random variables for the number of short and long epochs terminated at level $\ell$, respectively.
%By definition, we have $X_\ell = X^{short}_\ell + X^{long}_\ell$. Note   that $X^{long}_\ell \le 2t_\ell / (5^{\ell}/2) = 4t_\ell / 5^\ell$.

Write $\eta = 1/16e$, let $T'_\ell$ be the r.v.\ for the number of level-$\ell$ epochs that are $\eta$-short (hereafter, \emph{short}),
and let $T''_\ell = T_\ell - T'_\ell$ be the r.v.\ for the number of remaining level-$\ell$ epochs, i.e., those that are not short.
%let $B_\ell$ be the event that
%at least half of the $X_\ell$ natural epochs that are terminated at level $\ell$ are $\eta$-short,
%and
Let $A_\ell$ be the event that both $T_\ell > 4\log n$ and $T'_\ell \ge T_\ell / 4$  hold, or equivalently, $4T'_\ell \ge T_\ell > 4 \log n$.
\begin{claim} \label{first1}
$\Prob(A_\ell) \le 8/ (3n^4)$.
\end{claim}
\begin{proof}
Fix two parameters $q$ and $j$, with $j \ge q/4$,
and consider any $q$ level-$\ell$ epochs $E_1,\ldots,E_q$, ordered by their creation time, so that $E_i$ was created before $E_{i+1}$, for each $i = 1,2,\ldots,q-1$.
%and $E_q$ were created first and last among these $q$ epochs,
%respectively)
%among the $X_\ell$ natural epochs terminated at level $\ell$,

We argue that the probability that precisely $j$ particular epochs among these $q$ are short is bounded from above by $\eta^j$.
Indeed, by Corollary \ref{corborder}, the probability of an epoch to be short is at most $\eta$,
%even if it is given that the level of the epoch is $\ell$, and
independently of the uninterrupted durations of epochs that were creator prior to the current epoch's creation.
Thus, if we denote by $B^{(i)}$  the event that the $i$th epoch among these $j$ is short, for $1 \le i \le j$,
% (given that it is at level $\ell$ or regardless of this fact),
then we have  $\Prob(B^{(i)} ~\vert~ B^{(1)} \cap B^{(2)} \cap \ldots B^{(i-1)}) \le \eta$.
%(Moreover,
%$\Prob(A^{(i)} | A^{(1)} \cap A^{(2)} \cap \ldots A^{(i-1)})$ remains bounded by $\eta$
%this upper bound of $\eta$ on the probability continues to hold even if it is given that the $i$th epoch among these $q$, as well as any previously created epoch, is at level $\ell$.)
Consequently,
$$\Prob(B^{(1)} \cap B^{(2)} \cap \ldots \cap B^{(j)}) ~=~ \Prob(B^{(1)}) \cdot \Prob(B^{(2)} ~\vert~ B^{(1)}) \cdot \ldots \cdot \Prob(B^{(j)} ~\vert~ B^{(1)} \cap B^{(2)}
\cap \ldots B^{(j-1)}) ~\le~ \eta^j.$$

Next, we argue that $\Prob[T_\ell = q \cap T'_\ell = j] \le {q \choose j} \eta^j$.
%Instead of (i) going over all possibilities of choosing $q$ level-$\ell$ epochs among  all-level epochs,
%(ii) bounding the probability that each such possibility is chosen and precisely $j$ epochs out of the chosen $q$ are short,
%and (iii) taking the sum of all these probabilities, we handle all such possibilities \emph{together}. That is,
Indeed,  consider a sample space that consists of $q$ arbitrary level-$\ell$ epochs,
%denoted as above by $E_1,\ldots,E_q$, % denote the $q$ level-$\ell$ epochs,
%without actually choosing or fixing them among all epochs,
%and bound the probability that precisely $j$ of them are short.
%Specifically,   %(without actually choosing them among all-level epochs),
and note that there are ${q \choose j}$ possibilities to choose $j$ short epochs among them.   %$E_1,\ldots,E_q$.
As we have shown, each such possibility occurs with probability at most $\eta^j$, and the assertion follows.

%Hence $\Prob[X_\ell = q]$ is bounded from above by the probability that among $q$ epochs, at least $q/2$ of them have duration at most $2t_\ell/q$.
%Recall that the probability that any of these epochs has duration at most $2t_\ell/q$ is bounded by $2t_\ell/(q (5^\ell))$, independently of other epochs.

Noting that ${q \choose j} \le (eq/j)^j \le (4e)^j$ and recalling that $\eta = 1/16e$, we have ${q \choose j} \eta^j \le (1/4)^j$.
%for all $j$ and $q$ such that $j \ge q/2$,
Hence
%We have
\begin{eqnarray*}
\Prob(A_\ell) &=& \Prob[T_\ell  >  4\log n \cap T'_\ell \ge T_\ell / 4]
~=~ \sum_{q > 4 \log n} \sum_{j = q/4}^q \Prob[T_\ell = q \cap T'_\ell = j]
\\ &\le& \sum_{q > 4 \log n} \sum_{j = q/4}^q {q \choose j} \eta^j
~\le~ \sum_{q > 4 \log n} \sum_{j = q/4}^q (1/4)^j
~\le~
\sum_{q > 4 \log n} 4/3((1/2)^q)
\\ &\le& 8/3 ((1/2)^{4\log n}) ~\le~ 8/ (3n^4).
\end{eqnarray*}
\end{proof}

Let $c$ be a sufficiently large constant.
%\begin{claim} \label{suffice}
%If $\neg B_{\ell}$, then $Y_\ell < ct_\ell$.
%\end{claim}
%\begin{proof}
%\end{proof}
\begin{claim} \label{negate}
If $\neg A_{\ell}$, then $Y_\ell < c(t_\ell + 5^\ell \cdot \log n)$.
\end{claim}
\begin{proof}
First note that $Y_\ell = 0$, for any induced level $\ell$. We   henceforth assume that $\ell$ is a natural level.

If $\neg A_\ell$, then either $T_\ell \le 4\log n$ or $T'_\ell < T_\ell / 4$ must hold.

In the former case $X_\ell \le T_\ell \le 4\log n$, and we have $$Y_\ell ~=~ O(5^\ell) \cdot X_\ell ~\le~ O(5^\ell) \cdot  4\log n ~<~ c 5^\ell \cdot   \log n ~\le~ c(t_\ell + 5^\ell \cdot \log n).$$
Next, suppose that $T'_\ell < T_\ell / 4$.
In this case $T''_\ell > 3T_\ell/4$, i.e.,  more than three quarters of the $T_\ell$  epochs that are terminated at level $\ell$ are   not short.
Since $\ell$ is a natural level, at least half of the $T_\ell$ epochs are (fully-)natural.
In other words, $X_\ell \ge T_\ell/2$. It follows that at least a quarter of the $T_\ell$ epochs that terminated at level $\ell$ are both (fully-)natural and not short.
Denoting  by $X''_\ell$ the r.v.\ for the number of epochs that are both (fully-)natural and not short,
% denote the number of such epochs by $\tilde X_\ell$.
we thus have $X''_\ell \ge T_\ell/4 \ge X_\ell / 4$.
Since these $X''_\ell$ epochs are natural, the duration of each of them is equal to its uninterrupted duration, and thus it exceeds $\eta 5^\ell$.
Therefore, Observation \ref{obs:duration} yields $X''_{\ell} < 2t_\ell / (\eta 5^\ell)$.
% holds on the other hand.
We conclude that
$$Y_\ell ~=~ O(5^\ell) \cdot X_\ell ~\le~ O(5^\ell) \cdot 4X''_\ell ~\le~ O(5^\ell) \cdot 8t_\ell / (\eta 5^\ell) ~<~ ct_\ell ~<~ c(t_\ell + 5^\ell \cdot \log n). $$
%whereas in the latter case Claim \ref{suffice} yields $Y_\ell < ct_\ell$.
%
\end{proof}

Let $A$ be the event that $Y > c(t + (3/2) n\log n)$.
Claim \ref{negate} yields the following corollary.
\begin{corollary} \label{second2}
If $A$, then $A_0 \cup A_1 \cup \ldots A_{\log_5(n-1)}$.
\end{corollary}
\begin{proof}
%Suppose for contradiction that $A$ holds yet $A_0 \cup A_2 \cup \ldots A_{\log_5(n-1)}$ does not hold.
%In other words, we have
We assume that $\neg A_0 \cap \neg A_1 \cap \ldots \neg A_{\log_5(n-1)}$ holds, and show that $A$ cannot hold.
Indeed, by Claim \ref{negate}, we have that $Y_\ell < c(t_\ell + 5^\ell \cdot \log n)$ for each $\ell \ge 0$. It follows that
\begin{equation} \label{sumi}
Y ~=~ \sum_{\ell \ge 0} Y_\ell ~<~ \sum_{\ell \ge 0} c(t_\ell + 5^\ell \cdot \log n)  ~\le~ c(t + (3/2) n\log n). 
\end{equation}
%contradicting the fact that $A$ holds. 
\end{proof}

Claim \ref{first1} and Corollary \ref{second2} imply that
\begin{equation} \label{finall}
\Prob(A) ~\le~ \Prob(A_0 \cup A_1 \cup \ldots A_{\log_5(n-1)}) ~\le~ \sum_{\ell \ge 0} \Prob(A_\ell) ~\le~ (\log_5(n-1) + 1) (8/ (3n^4)) ~=~ O(\log n / n^4).
\end{equation}
It follows that $Y$ is upper bounded by $O(t + n\log n)$ with high probability, as required.
%We use the following claim to prove .
%\begin{claim} \label{claim:basic}
%For any $q > 1$, $\Prob[X_i = q] \le \sum_{j = q/2}^q \left(\frac{4et_i}{q (5^i)}\right)^j$.
%\end{claim}
%\begin{proof}
%Fix any $q > 1$.
%If $q$ level-$\ell$ epochs are terminated during $t_\ell$ edge deletions, at least half of them have duration at most $2t_\ell/q$.
%It follows that
\ignore{
\begin{eqnarray} \label{claim:basic}
\Prob[X_\ell = q] &\le& \sum_{j = q/2}^q {q \choose j} \left(\frac{2t_\ell}{q (5^\ell)}\right)^j ~\le~
%\sum_{j = q/2}^q \left(\frac{eq}{j}\right)^j \left(\frac{2t_i}{q (5^i)}\right)^j
%\\ &\le&
\sum_{j = q/2}^q (2e)^j \left(\frac{2t_\ell}{q (5^\ell)}\right)^j
~=~ \sum_{j = q/2}^q \left(\frac{4et_\ell}{q (5^\ell)}\right)^j.
\end{eqnarray}

%
%\end{proof}
%We proceed with the proof of Lemma \ref{prob}.

Set $q_0 = 4(4et_\ell/5^\ell + \log n)$.
For any $q > q_0$, we have $\Prob[X_\ell = q] \le 4/3((1/2)^q)$ by (\ref{claim:basic}).
Therefore $$\Prob[X_\ell > q_0] ~=~ \sum_{q > q_0} \Prob[X_\ell = q] ~\le~ \sum_{q > q_0} 4/3((1/2)^q) ~\le~ 8/3 (1/2)^{q_0} ~<~ 8/3 (1/2)^{4\log n} ~=~  8/ (3n^4).$$
Thus $X_\ell$ is bounded by $O(t_\ell / 5^\ell + \log n)$ with high probability, as required.}

\subsection{Expected bound} \label{justify}

\ignore{
%\end{proof} completing the proof of Lemma \ref{prob}
\subsection{Justifying the assumption} \label{justify}
Consider any level $\ell$ where our assumption does not hold, i.e.,  $T_\ell > 2X_\ell$,
%We claim that such levels can be disregarded from the runtime analysis.
whence the number of induced epochs terminated at level $\ell$ exceeds the number of natural epochs terminated at that level.
Next, we show that the computation costs incurred by level $\ell$ can be charged to the computation costs at higher levels,
allowing us to disregard any level where the assumption does not hold in the runtime analysis.
%ded from the runtime analysis. More accurately, we will charge the

As $T_\ell > 2X_\ell$,
we may define a one-to-one mapping from the natural to the induced epochs, mapping each natural level-$\ell$ epoch to a unique induced epoch at that level.
Then we can (temporarily) charge the costs of any level-$\ell$ natural epoch to the induced epoch to which it is mapped.
In Section 3.3, we defined the recursive cost of  an epoch as the sum of its actual cost and the recursive costs of the at most two induced
epochs (at lower levels) terminated by it. Let us re-define the recursive cost of an epoch
as the sum of its actual cost and the recursive costs of the at most two induced epochs terminated by it as well as the at most two natural epochs
%to which the induced epochs are charged.
%that
corresponding to them under the aforementioned mapping. 
%i.e., those whose costs are charged to the terminated induced epochs.

We henceforth change the constant 3 to 5 throughout the paper; in particular, instead of using $\log_5(n-1)$ levels, we will use $\log_5(n-1)$ levels.
Consequently, we allow the computation cost associated with any level-$\ell$ epoch to grow from $O(5^\ell)$ to  $O(5^\ell)$ (cf.\ Lemma \ref{basiccost}),
and obtain the recurrence $\hat C_{\ell} \le   4 \hat C_{\ell-1} + O(5^{\ell})$,
with the base condition
$\hat C_{0} =  O(1)$, which resolves to $\hat C_{\ell} = O(5^{\ell})$ (cf.\ Corollary \ref{important}).
}


\section{Improving the high probability bound} \label{app:improve}
%\vspace{10pt}
%\noindent
If the length $t$ of the update sequence is $\Omega(n \log n)$, then our current high probability runtime bound  $O(t + n \log n)$ reduces   to $O(t)$.
It is natural to assume that $t \ge n/2$, otherwise some vertices are ``idle'', and we can simply ignore them.
%\footnote{
(Such an assumption needs to be properly justified.
%(E.g., the algorithm of \cite{BGS11} maintains an array of size $\log_2 n$ for each vertex $v$ with the values of $\phi_v(j)$, $j = 0,\ldots,\log_2 n$,
%and it needs to be adapted accordingly.)
Nevertheless, dropping it usually triggers only minor adjustments.)
%}
One may further assume that $t =  \Omega(n \log n)$, as this is indeed the case in many practical applications.
However, we believe that it is important to address the regime $n/2 \le t = o(n \log n)$, for both theoretical and practical reasons.
%Furthermore, even the fact
%Although in many practical applications it indeed holds that $t = \Omega(n \log n)$, the case of shorter update sequences should not be ignored.


%In any case, one may not assume that $t = \omega(n)$.
We do not make any assumption on $t$.
%This assumption may lose generality, as
%Nevertheless, some algorithms need to know how many vertices are involved.
%Often this only leads to minor adjustments.
%but that's not the case in our algorithm if I understand correctly.)
%Baswana et al.\ \cite{BGS11} showed a total runtime bound of $O(t \log n + n \log^2 n)$.
For $t = \Omega(n^\eps)$, we prove that the runtime exceeds $O(t)$ with probability (w.p.) polynomially small in $n$.
For smaller values of $t$, we  prove that the runtime exceeds $O(t)$ w.p.\ polynomially small in $t$.
Note that in the latter regime most of the $n$ vertices are idle,  and it does not make much sense that this probability would depend on the number of idle vertices;
nevertheless, for completeness, we show that the runtime exceeds $O(t + \log n \cdot \sqrt{t})$ w.p.\ polynomially small in $n$.
%However, in order to improve it to $O(t)$, we need the
%) to $O(t)$, . Our goal is to improve it to $O(t)$,
%which implies shaving a factor of $n \log n/ t$ in the regime $t = o(n\log n)$.  %, and  a larger factor if $t = o(n)$.

Let us revisit some of the details in the proof of Lemma \ref{expect}(2).
Recall that $A_\ell$ is the event that both $T_\ell > 4\log n$ and $T'_\ell \ge T_\ell / 4$  hold.
Instead, let us re-define $A_\ell$ to be the event that both $T_\ell > 4\log t$ and $T'_\ell \ge T_\ell / 4$  hold.
This modification triggers several changes.
First, Claim \ref{first1} will change to $\Prob(A_\ell) \le 8/ (3t^4)$.
Second, Claim \ref{negate} will be changed, so that if $\neg A_\ell$, then $Y_\ell < c(t_\ell + 5^\ell \cdot \log t)$.

In exactly the same way as before, we will be able to argue that $Y$ exceeds $O(t + n \log t)$ with probability $O(\log n / t^4)$.
However, this high probability bound is not what we are looking for.
% -- we want to have $Y$ bounded by $O(t)$ with probability
%if $\neg A_\ell$, then $Y_\ell < c(t_\ell + 5^\ell \cdot \log n)$.
%The second assertion of Lemma \ref{expect} states that
%the number $X_\ell$ of natural epochs terminated at level $\ell$ is $O(t_\ell / 5^\ell + \log n)$ w.h.p., specifically,
%$X_\ell$ exceeds this bound w.p.\ $O(n^{-4})$.
%In exactly the same way we have  that $X_\ell$ exceeds $O(t_\ell / 5^\ell + \log t)$ w.p.\ $O(t^{-4})$.
%As the recursive cost associated with any level-$\ell$ epoch is $O(5^\ell)$, the total cost associated with all natural level-$\ell$ epochs exceeds
%$O(t_\ell + \log t \cdot 5^\ell)$ w.p.\ $O(t^{-4})$.

The key insight for improving the high probability bound is given by the following lemma.
\begin{lemma} \label{maining}
%guarantee that the maximum level of any vertex will be much smaller than $\log 3 (n-1)$.
%Specifically, we do not allow
The level of all vertices can be bounded by $\log_5 (2\sqrt{t})$, while increasing the total runtime of our algorithm by at most a constant factor.
\end{lemma}
%The first suggestion might be to try guaranteeing that all out-degrees will be small w.r.t.\ $t$, namely, at most $c \sqrt{t}$, for an appropriate constant $c$.
Before proving this lemma, we demonstrate its power.
That is, we assume that the level of all vertices is bounded by $\log_5 (2\sqrt{t})$ and that the runtime required for that is negligible,
and show that the high probability bound can be improved under this assumption.
(Notice that we do not attempt to bound the out-degree  of vertices by $2\sqrt{t}$.)
In this case Equation (\ref{sumi}) in the proof of Corollary \ref{second2} will be changed to
$$Y ~=~ \sum_{\ell = 0}^{\log_5 (2\sqrt{t})} Y_\ell ~\le~ \sum_{\ell = 0}^{\log_5 (2\sqrt{t})} c(t_\ell + 5^\ell \cdot \log t)  ~\le~ c(t + (3/2) 2\sqrt{t} \log t).$$
Consequently, we can re-define $A$ to be the event that $Y > c(t + (3/2) 2\sqrt{t}\log t)$, without affecting the validity of Corollary \ref{second2}.
Finally, Equation (\ref{finall}) will be changed to
$$\Prob(A) ~\le~ \Prob(A_0 \cup A_1 \cup \ldots A_{\log_5 (2\sqrt{t})}) ~\le~ \sum_{\ell = 0}^{\log_5 (2\sqrt{t})} \Prob(A_\ell) ~\le~ (\log_5(2\sqrt{t}) + 1) (8/ (3t^4)) ~=~ O(\log t / t^4).$$
%\end{equation}
Thus, assuming the level of vertices is bounded by $\log_5 (2\sqrt{t})$,
$Y$ exceeds $c(t + (3/2) 2\sqrt{t}\log t) = O(t)$ w.p.\ $O(\log t/t^4)$, which is polynomially small in $t$ for all  $n$ and $t$
and polynomially small in $n$ for all $t = \Omega(n^\eps)$.

%summing over all possible levels $\ell = 0,1,\ldots,\log_5 (2\sqrt{t})$ of epochs,
For the somewhat degenerate regime $t = o(n^{\eps})$, we simply use the original events $A_\ell$ and the original claims
(Claim \ref{first1} and \ref{negate}). Since the number of levels is bounded by $\log_5 (2\sqrt{t})$,
Equation (\ref{sumi}) in the proof of Corollary \ref{second2} will be changed to
$$Y ~=~ \sum_{\ell = 0}^{\log_5 (2\sqrt{t})} Y_\ell ~\le~ \sum_{\ell = 0}^{\log_5 (2\sqrt{t})} c(t_\ell + 5^\ell \cdot \log n)  ~\le~ c(t + (3/2) 2\sqrt{t} \log n).$$
Consequently, we can re-define $A$ to be the event that $Y > c(t + (3/2) 2\sqrt{t}\log n)$, without affecting the validity of Corollary \ref{second2}.
Finally, Equation (\ref{finall}) will be changed to
$$\Prob(A) ~\le~ \Prob(A_0 \cup A_1 \cup \ldots A_{\log_5 (2\sqrt{t})}) ~\le~ \sum_{\ell = 0}^{\log_5 (2\sqrt{t})} \Prob(A_\ell) ~\le~ (\log_5(2\sqrt{t}) + 1) (8/ (3n^4)) ~=~ O(\log t / n^4).$$
%\end{equation}
Thus, assuming the level of vertices is bounded by $\log_5 (2\sqrt{t})$,
$Y$ exceeds $c(t + (3/2) 2\sqrt{t}\log n) = O(t +   \log n \cdot \sqrt{t})$ w.p.\ $O(\log t/n^4)$, which is polynomially small in $n$ for all $t = o(n^\eps)$.
\vspace{10pt}
\noindent
\\
{\bf Proof of Lemma \ref{maining}:}
\vspace{3pt}
\\
%Consider a vertex of level lower than $\ell_{max} = \log_5 \sqrt{t}$ that becomes temporarily free.
Upon re-evaluating the level of a vertex, our algorithm may increase its level beyond $\ell_{max} := \log_5 (2\sqrt{t})$, as part of the rising process that creates
a new epoch of sufficiently high level, within Procedure $\rand$.
We adjust Procedure $\rand(v)$   by preventing $\ell^*$ from growing beyond $\ell_{max}$.
Specifically, we execute the loop in line 2 of the procedure as long as $\ell^* < \ell_{max}$, or in other words,
we adapt the continuation condition $\phi_v(\ell^*+1) \ge 5^{\ell^*+1}$ of the while loop to be $\phi_v(\ell^*+1) \ge 5^{\ell^*+1}$ and $\ell^* < \ell_{max}$.
%, we set $\ell^*$ to be $\min\{\ell_{max},\ell^*\}$.
As a result, we can no longer argue that the resulting level $\ell^*$ satisfies $\phi_v(\ell^*+1) < 5^{\ell^*+1}$.
While this upper bound on $\phi_v(\ell^*+1)$ may no longer hold,
%, namely $\phi_v(\ell^*+1) < 5^{\ell^*+1}$,
note that the lower bound on $\phi_v(\ell^*)$, namely $\phi_v(\ell^*) \ge 5^{\ell^*}$, remains valid (cf.\ Lemma \ref{rand_basic}(3)).
The next observation thus follows from Corollary \ref{Ob:basic}.
\begin{observation} \label{obs:init}
Any vertex initiating a level-$\ell_{max}$ epoch has out-degree at least $5^{\ell_{max}} = 2\sqrt{t}$ at that time.
In particular, at least this number of edges incident on such a  vertex were inserted to the graph.
%(We stress that our adjustments may weaken the upper bound on the out-degree of such a vertex, but the lower bound remains valid.)
\end{observation}
%\begin{proof}
%As before, after the call to $\setlvl(v,\ell^*)$, all outgoing neighbors of $v$ are of level strictly lower than $\ell^*$.

As before, the mate $w$ of $v$ is chosen uniformly at random among $v$'s outgoing neighbors, and $\ell_w < \ell^*$.
More accurately, as detailed below, in some cases we restrict our attention to a \emph{subset} of $v$'s outgoing neighbors,
and choose the mate $w$ of $v$ uniformly at random among the vertices of this subset.
However, in any case, it is guaranteed that the level of $v$'s random mate $w$ will be strictly lower than that of $v$.

Another adjustment is to skip line 9 of Procedure $\rand(v)$ if $\ell^* = \ell_{max}$; indeed, if the new epoch is of
  level  $\ell_{max}$, we cannot make a recursive call that creates an epoch at   a higher level.
%is to remove line (9) of
%Even though the test in line (9) of Procedure $\rand(v)$ may check positive, we do not terminate the newly created epoch corresponding to edge $(v,w)$,
%but rather jump to line (!0) of the procedure.
%This inequality is violated only when $\ell^* = \ell_{max}(t)$.

%In what follows assume that $\ell^* = \ell_{max}(t)$.

Note that the calls to $\setlvl(v,\ell^*)$ and $\setlvl(w,\ell^*)$ do not effect the incoming neighbors of $v$ and $w$ with maximum level $\ell_{max}$,
which   remain incoming to them after the calls.
%all these incoming neighbors of $v$ and $w$ will remain incoming to them after the calls.  %se calls do not flip the corresponding edges.
%calls do not flip any incoming edges from these neighbors.
Consequently, for any vertex of level $\ell_{max}$, all its outgoing edges do not flip.
%Note also that for any such vertex, all its incoming edges must be from vertices of maximum level $\ell_{max}$,
%implying that its incoming edges do not flip as well.
Suppose that the new matched edge $(v,w)$ is of maximum level $\ell_{max}$, and consider the newly created epoch corresponding to it.
Since we guarantee that a random mate has a strictly lower level than the vertex choosing it,
the endpoints $v$ and $w$ of this epoch cannot be chosen as random mates of any vertex during the epoch's lifespan,
implying that such an epoch can be terminated only by deleting its associated edge $(v,w)$ from the graph.  %adversarial edge deletions.
Thus any epoch of maximum level is a natural epoch, and all edges that are outgoing of its endpoints do not flip.
%some of the edges that are incoming
%to its endpoints may
We have shown that, once a vertex rises to level $\ell_{max}$, the epoch associated with it becomes somewhat ``stagnant''.
% all the edges incident on the endpoints of any such epoch preserve their orientation
%throughout the
%Thus, from the moment an epoch at level $

Lemma \ref{rand_basic} implies that the runtime of the call to $\setlvl(v,\ell^*)$ (respectively, $\setlvl(w,\ell^*))$ is
$O(\dout(v) + \ell^*) = O(\dout(v))$ (resp., $O(\dout(w) + \ell^*) = O(\dout(w))$),
where $\dout(v) = \phi_v(\ell^*)$ (resp., $\dout(w) = \phi_w(\ell^*)$) is the new out-degree of $v$ (resp., $w$).
However, if $\ell^* = \ell_{max}$, we may not be able to upper bound neither $\dout(v)$ nor $\dout(w)$ by $O(5^{\ell^*}) = O(\sqrt{t})$.
Suppose w.l.o.g.\ that $\dout(v)  \ge \dout(w)$.
If $\dout(v) = O(5^{\ell^*})$, then our original analysis carries through.
We henceforth assume that $\ell^* = \ell_{max}$ and $\dout(v) := D \gg \sqrt{t}$, and show how to charge this $O(D)$ cost without creating an epoch at a higher level.
%The original procedure compensates for this cost by making a recursive call which creates an epoch at level higher than $\ell^*$;
%however, in the case that $\ell^* = \ell_{max}(t)$, we cannot make such a call.


%Assume that $\ell^* = \ell_{max}(t)$.
%Note that for any vertex of level $\ell_{max}(t)$, none of its incident edges will be


Consider the next time  that vertex $v$ becomes temporarily free, and denote by $\dout^{new}(v)$ the out-degree of $v$ at that time.
As mentioned, $v$ may become temporarily free only as a result of its matched edge $(v,w)$ being deleted from the graph, which terminates the corresponding level-$\ell_{max}$ epoch.
Since $v$ has become temporarily free, our update algorithm handles it by invoking Procedure $\evalf(v)$.
%and recall that $D$ denotes $v$'s out-degree at the time the corresponding level-$\ell_{max}(t)$ epoch was created.
%Moreover, the new out-degree $\dout^{new}(v)$
%terminated, due to the deletion of edge $(v,w)$.

If $\dout^{new}(v) < 5^{\ell_{max}+1} = 6\sqrt{t}$,     Procedure $\evalf(v)$ calls to $\detr(v)$.
Due to the stagnation properties discussed above, all outgoing edges of $v$ at the time the epoch was created do not flip until its termination.
Hence, $D - \dout^{new}(v) = \Omega(D)$ edges incident on $v$  must have been deleted from the graph during this time interval,
and we can charge the original $O(D)$ cost to these edge deletions.

In the complementary case $\dout^{new}(v) \ge 5^{\ell_{max}+1} = 6\sqrt{t}$, this procedure calls to $\rand(v)$.
We make another adjustment to Procedure $\rand(v)$ for this particular case.
% where the examined vertex $v$ is of maximum level $\ell_{max}(t)$
%and $\dout^{new}(v) > 5^{\ell_{max}(t)+1} = 3\sqrt{t}$.
Specifically, in this case the procedure scans $3\sqrt{t}$ arbitrary outgoing neighbors of $v$,
and picks a mate $\tilde w$ for $v$ uniformly at random among $v$'s scanned neighbors that are of level strictly lower than $\ell_{max}$.
%the next observation shows that there are at least $\sqrt{t}$ such neighbors.
The level of $v$ remains $\ell_{max}$, and the level of $\tilde w$ is set to $\ell_{max}$ by calling   $\setlvl(\tilde w, \ell_{max})$, thus creating a level-$\ell_{max}$ epoch.
%that there are at least $2\sqrt{t}$ of them.
%Note that we, however, that this call will create an epoch at level higher than $\ell_{max}(t)$.
%To this end we make the following key observation. % is that
\begin{claim} \label{Obs:key}
For any vertex $v$,
at most $2\sqrt{t}$ of its neighbors may have level $\ell_{max}$ at any   point in time.
%at most $\sqrt{5^{i-1}}$ of its neighbors may have performed a special reset within the current time interval.
\end{claim}
\begin{proof}
%By the description of the algorithm, the level of a vertex may increase to $\ell$, where $\ell >0$ is an arbitrary parameter, only if this vertex initiates the creation of a new %epoch at level $\ell$,
%or is chosen as a random mate of such a vertex.
%where $\ell >0$ is an arbitrary parameter.
%By the above description, a vertex performs a special reset only after it makes a failed attempt to initiate the creation of an epoch at level greater than
%the required threshold $\ell_{max}(5^{i-1})$. %, which is terminated.
%Consequently, any vertex that performs a special reset within this time interval has out-degree greater than $c \sqrt{5^{i-1}}$ at the time of the reset.
Suppose for contradiction that more than $2\sqrt{t}$ neighbors of some vertex $v$ have level $\ell_{max}$ at some point in time.
Each of these neighbors is part of a single level-$\ell_{max}$ epoch at that time,
and the edges corresponding to these epochs are vertex-disjoint.
In particular, at least half of these neighbors of $v$ must have initiated a level-$\ell_{max}$ epoch,
or in other words, more than $\sqrt{t}$ vertices must have initiated a level-$\ell_{max}$-epoch.
%were to perform a special reset within the current time interval,
Observation \ref{obs:init} implies that the total number of edges ever incident on those vertices exceeds $(\sqrt{t} \cdot 2\sqrt{t})/2 = t$,
contradicting the fact that the total number of edge updates is $t$.
%edges ever inserted to the graph
\end{proof}
Claim \ref{Obs:key} implies
%the procedure will match $v$ to some random neighbor of level strictly lower than $\ell_{max}(t)$
that $v$'s mate $\tilde w$ is chosen with probability at most $1/\sqrt{t}$. A key property is that the runtime $O(\sqrt{t})$ of Procedure $\rand(v)$ in this case does not depend on
$v$'s out-degree.
%specifically, it is $O(\sqrt{t})$.  % which is at most inverse-linear to the probability in which the matched edge is chosen.

To summarize, the original $O(D)$ cost needed for rising a vertex $v$ to the maximum level $\ell_{max}$ is linear in the out-degree of $v$ at that time,
which may be prohibitively large.
However, the runtime of subsequent calls to Procedure $\rand(v)$ is $O(\sqrt{t})$, which is inverse-linear in the probability with which the matched edge is chosen,
and then our original analysis carries through. Since the level of $v$ remains $\ell_{max}$ in all such calls to Procedure $\rand(v)$,
the original $O(D)$ cost can be charged to the insertions of the $D$ outgoing edges of $v$ at that time.
% corresponding edge flips.
On the other hand, if a subsequent call to Procedure $\detr(v)$ is made, then $v$'s level will decrease to $-1$ or 0,
which implies that we may have to spend an additional prohibitively large cost to rise $v$ to the maximum level $\ell_{max}$ in the future.
%with $D'$ being a possibly different parameter than $D$.
However, at least $\Omega(D)$ edge deletions incident on $v$ must have occurred until that time, to which we can charge the original $O(D)$ cost,
and then this charging argument can be reapplied from scratch.

This completes the proof of Lemma \ref{maining}. 

%\vspace{-4pt}
\section{Applications} \label{app:app}
%\vspace{-2pt}
{\bf Dynamic approximate MWMs.~}
As mentioned, Anand et al.\ \cite{ABGS12} gave a randomized algorithm for maintaining an 8-MWM in general $n$-vertex weighted graphs with expected update time $O(\log n \log \Delta)$.
% where $\Delta$ is the ratio between
%the maximum and minimum edge weights in the graph.
Their algorithm maintains a partition of the edges in the graph into $O(\log \Delta)$ buckets according to their weight, with each bucket containing
edges of the same weight up to a constant factor. The maximal matching algorithm of \cite{BGS11} is employed (as a black-box) for each bucket separately.
By  carefully maintaining a matching in the graph obtained from the union of these $O(\log \Delta)$ maximal matchings, an 8-MWM is maintained in \cite{ABGS12}.
%employs the dynamic maximal matching algorithm of \cite{BGS11} as a black-box.
By plugging our improved algorithm, we   shave a factor of $\log n$ from the update time.
%Thus, we obtain an algorithm for maintaining an 8-MWM
%in general weighted graphs with expected update time $O(\log \Delta)$.
\begin{theorem}
Starting from an empty graph on $n$ fixed vertices, an 8-MWM can be maintained over any sequence of edge insertions and deletions
in expected amortized update time $O(\log \Delta)$, where $\Delta$ is the ratio between the maximum and minimum edge weights in the graph.
%For any update sequence of length $t$ that start from an empty graph, there is a randomized algorithm for maintaining a maximal matching within total expected time $O(t)$.
%The time bound holds with high probability, and the space usage of the algorithm is
%$O(n +m)$, where $n$ is the fixed number of vertices and $m$ is the constantly changing number of edges.
\end{theorem}
\vspace{4pt}
{\bf Distributed networks.~} Consider an arbitrary sequence of edge insertions and deletions in a distributed network.
%In order to find a free neighbor of some vertex $v$,
%the algorithm scans all neighbors of $v$ until a free neighbor is found.
Note that each vertex $v$ can gather complete information about its neighbors in two communication rounds.
Consequently, the na\"{\i}ve  (centralized) maximal matching algorithm discussed in Section 1.4 can be distributed in the obvious way,
requiring $O(1)$ communication rounds following a single edge update.
Moreover, messages of size $O(\log n)$ suffice for communicating the relevant information.
%Following an edge update, if the matching was maximal, then a single communication round suffices for updating it to be maximal again.
%It is thus immediate to obtain a distributed algorithm for maintaining a maximal matching (and thus 2-MCM and 2-MCVC) with a single communication round per update.
On the negative side, the number of messages sent per update may be as high as $O(n)$.
Note, however, that the total number of messages sent is upper bounded (up to a constant) by the total number of neighbor scans performed by the centralized algorithm.
%(and is therefore also bounded by the total runtime of the centralized algorithm).
This phenomenon extends far beyond the na\"{\i}ve maximal matching algorithm. In particular, it holds also w.r.t.\ Baswana et al.'s algorithm \cite{BGS11} and our algorithm.
Our analysis of Section \ref{sec:mainanal} shows that the amortized update time is constant,  %$O(1)$ both in expectation and w.h.p.
thus the average number of neighbor scans is also a  constant. (We did not try to optimize the latter constant, but it is rather small.)
%It follows that the average number of messages sent
%and this phenomenon holds in general: Any
%We demonstrate that our dynamic maximal matching algorithm can be easily distributed, so that the average number of messages sent per update is a small constant.
%Next, we upper bound the total number of neighbor scans performed by our algorithm.
%Consider a vertex $v$ that becomes temporarily free. If $\dout(v) \le 5^{\ell_v+1}$, then Procedure $\detr$ is invoked.
%In this case, at most $5^{\ell_v+1}$ neighbor scans are performed, and they are charged
\begin{theorem}
Starting from an empty distributed network on $n$ fixed vertices, a maximal matching (and thus 2-MCM and also 2-MCVC)
can be maintained distributively (under the $\mathcal{CONGEST}$ communication model) over any sequence of edge insertions and deletions with a constant amortized \emph{message complexity}.  % of a constant. % most 76.
\end{theorem}
{\bf Remark.} Optimizing the constant behind the amortized message complexity is left as an open question.

}

\ignore{
\clearpage

\section{Junk}
%[[S:  say that our algorithm is inherently simpler?  Maybe add  better and simpler to the title]]
[[S: Make sure to address the issue of level-1 matched edges]]
[[S: saving space: first paragraph of Sect. 2, the data structure section 3.1 (boring), Sect. 2.3.
Recall: I left the first paragraph in ``Baswana et al.'s scheme'' (in the technical overview section), can remove it.
Other places to save space: The footnote description on [AV-W14], the footnote on adversarial model.
Also: first sentence of ``wrapping up''. Maybe squeeze ack to one line.
Maybe can remove Lemma 3.4? don't think so... (but need to move backwards, to after Claim 3.2.
Should save space in applications. Remove some stuff from 1.3 (as it appears already in 1.4, and if not, then move there),
and then remove Organization part. I would also remove a line in Section 3.1]]

%[[S: maybe specify the constant (the number of neighbors scanned at each step on average)]]

%[[S: maybe give application to distributed networks, the message complexity. Upper bound the amortized message complexity, specify constants]]

%[[S: maybe our storage can be made linear, whereas their storage is at least nlogn (or maybe even quadratic?, don't think so)]]

%[[S: maybe we can claim w.h.p. constant, even when the length of the sequence is small. In that regime, I think they got $\log^2 n$ bound]]

%\paragraph{junk}
%Define $d_i(v)$ to be the number of neighbors of $v$ whose level is at most $i$.
%[[S: let's use $\phi_v(i+1)$ instead, to be in accordance with their notation.]]

%[[S: DEL: If $j$ denotes the previous level of $v$, then if the number of outgoing neighbors is $O(2^j)$,
%we can pay for the evaluation from the old potential. But otherwise, the new level of $v$ will be greater than $j$, in which case
%the eval cost will be paid by the new epoch, which will correspond to level $\tilde j > j$.]]

[[S: DEL: Also need to say that there are no edges between level-0 vertices, meaning that whenever the level of a vertex increases from -1 to 0 (turns from free to matched),
there is no violation, because all its incoming neighbors must be of level at least 0.]]


[[S: I don't mind having a too-large estimation on the level,
but I don't want to have a too-small estimation, and then to pick it randomly as a low-level vertex
only to find out (after evaluating its level) that its true level is larger than that.
(NOTE HOWEVER THAT THIS IS THE SITUATION ANYWAY... WE CAN'T CHANGE THIS)
If the estimation is too large, the only problem is to miss in this way a free vertex (whose level should be 0), but if we make sure to handle
those free vertices later (after evaluating their level as 0), then there is no problem.]]

[[S: choose one among $i$ and $\ell$ and be consistent, maybe add $j$ or other parameters]]

[[S: after Lemma 3.4]]
The key idea behind our charging scheme %intuition as to why Lemma \ref{basiccost} is true
can be summarized as follows.
Consider a vertex $v$ that becomes temporarily free. If its out-degree is ``small'' (w.r.t.\ $5^{\ell_v}$), then we handle $v$ deterministically
and charge this cost to the past (i.e., to the termination cost of the corresponding level-$\ell_v$ epoch).
The interesting case is when the out-degree of $v$ is ``large'' (w.r.t.\ $5^{\ell_v}$), and then $v$ should rise to a higher level.
Since the outgoing neighbors of $v$ are of level at most $\ell_v$ and since we have complete information of $v$'s incoming neighbors,
we can compute the appropriate level $\ell^*$ to which $v$ should rise, and also flip the edges incident on $v$ accordingly, in time $O(5^{\ell^*})$; see Lemma \ref{rand_basic}(4).
Moreover, by Lemmas \ref{rand_basic}(2) and \ref{rand_basic}(3), after $v$ rises to level $\ell^*$, it has at least $5^{\ell^*}$ outgoing neighbors of level strictly lower than $\ell^*$.
Thus, by choosing one of them uniformly at random as a mate for $v$, the matched edge is chosen with probability at most $1/5^{\ell^*}$.
Consequently, we can charge this cost of $O(5^{\ell^*})$ to the future (i.e., to the creation cost of the corresponding level-$\ell^*$ epoch),
as the new epoch can cover this cost in the amortized sense.
}

\ignore{
\paragraph{important for talk}
It is difficult to orient edges according to out-degree. Because following a single edge flip, there may be a long and chaotic ``wave''.
What they suggested is to preserve the out-degree up to some small factor. This is still quite difficult.
What i suggest is different. I orient according to levels, but levels don't represent the out-degree. In this way I can be lazy.
Then when I need to handle a vertex of large out-degree, I simply raise its level, and pick at random a neighbor to pay for it.

The key idea is this -- if I scan a certain neighbor, then I will make sure, when choosing a random neighbor, to include it as one of the neighbors.

For the talk, think of a wave. It takes a logarithmic time to raise it up to a certain level, and then it fades away for free.
Instead, we don't raise the wave to any level, waves can grow without any control.

Oh, I disregarded all the issue of induced deletions. This is a pity. When choosing a random mate that is matched,
I need it to have a much lower out-degree


%\paragraph{more junk}
The algorithm of BGS11 partitions the vertices into $\log n$ levels, and the time needed to handle each level is constant,
which gives the $O(\log n)$ time. Maybe I can mention that it's not that just the average time is logarithmic, it is usually at least so due to
updating a logarithmic number of entries in the underlying array.
It is natural to work with $\log_k n$, for a larger $k$. Then the number of levels can be significantly reduced.
However, the time needed to handle each level will be $O(k)$, which gives an update time of $O(\log_k n \cdot k)$, optimized when $k = O(1)$.

I would say that the main difference is that BGS11 aims to rise to the highest possible level, constantly and persistently,
whereas we try to rise to the lowest possible level, and just at the time we handle the vertex. The fact that a vertex cannot rise to a higher level
(by their approach) immediately implies that the out-degree is small. But much more than that, it implies that whenever the level of a vertex falls
by one unit, the levels of its neighbors will not rise to a higher level. (When the level of a vertex rises, no other vertex is affected.)
So they get a fading wave phenomenon. But in order to do that, they have to spend a lot of time (and space) for determining the highest possible level.
Moreover, the fading wave phenomenon is somewhat complicated, in terms of implementation, but also conceptually.
As a result of our lazy approach, we can't say anything on the out-degree, except for immediately after evaluation. In fact, even immediately after evaluation,
we don't say anything (due to deterministic settle, which sets the level to 0 but don't flip the edges towards level-0 vertices). While we can overcome this issue,
there is absolutely no need. Whenever we handle a vertex, the time we spent can be covered either by the previous matched edge incident on it or the new one that we will next create. I think the key insight is that if a guy has large degree, then its out-degree may get bigger and bigger, but the bigger it gets the more tokens we should acquire,
and eventually we are prone to stop because the degree is at most $n-1$, hence the level cannot grow beyond $\log_5 (n-1)$.

%Paraphrasing, they defined $\phi_v(j)$ to be the number of $v$'s neighbors with level smaller than $j$, for any $j > \ell_v$.
%Their requirement is that $\phi_v(j) < 2^j$ for any such $j$, otherwise the level of $v$ ``rises'' to the highest possible level for which the requirement is violated.
%(The rise of a vertex cannot cause another vertex to rise.)
%In particular, they ensure that the out-degree of any $j$-level vertex is smaller than $2^j$.

Maybe there's a chance to get worst-case bounds:  Worst-case update time of $f(eps)$ (say $O(1/\eps)$), with an approximation factor w.h.p.\ $2+\eps$.
I don't know if this is worth the effort.
}
\end {document}



